Gaia predicted brown dwarf detection rates around FGK stars in astrometry, radial velocity, and photometric transits

Context: The current sample of known brown dwarfs (BDs) around FGK-stars is only of the order of a hundred. The ongoing ESA mission Gaia has already collected its nominal 5 yr of mission data and might operate up to 10 yr. Aims: Using detailed simulations, we estimate the number of BDs that could be discovered by Gaia astrometry, radial velocity, and photometric transits around main sequence (V) and subgiants (IV) FGK host stars for a 5 and 10-yr mission. Methods: Using a robust $\Delta \chi^2$ statistic we analyse the BD companion detectability from the Besan\c{c}on Galaxy population synthesis model complemented by Gaia DR2 data for the bright end, using the latest Gaia performance and scanning law, and literature-based BD-parameter distributions. Results: We report here reliable detection numbers ($\Delta \chi^2$>50) for a 5-yr [10-yr] mission. Astrometry alone yields 28,000-42,000 [45,000-55,000] detections out to several hundred pc [>kiloparsec], with the majority around G magnitude 14-15 [14-16] and P>200 d. Gaia radial velocity time series allow detection of 830-1100 [1500-1900] mainly massive BDs (55-80 M_J), most having P <10 d. Systems with at least 3 photometric transits (S/N>3) are expected for 720-1100 [1400-2300] BDs, averaging at 4-5 [5-6] transits per source. Overlap of astrometric and radial velocity detection yield 370-410 [870-950] candidates, transit and radial velocity 17-27 [35-56], and transit and astrometric detection 1-3 [4-6]. Conclusions: Though above numbers have +/- 50% uncertainty due to the uncertain occurrence rate and period distribution of BDs around FGK host stars, Gaia detections will number in the tens-of-thousands, enlarging the current sample by at least two orders of magnitude, allowing to investigate the BD fraction and orbital architectures as a function of host stellar parameters in greater detail than every before.

==> Sec_BdDistribution.tex <==
%\subsection{Current models \label{sec:currentModel}}
%\subsection{Latest model \TODO{[set name]} \label{sec:latestModel}}
%As basis for our simulation we use the latest estimates from ....



==> figures/AuthorsAndAffiliations.tex <==
% TODO:
%- check some authors, 
%- leanne in wp leaders group 
% -inverse alphabetic for 4rd group and down?, 
% - some excluded authors correctly excluded?
% - ask CU5 to include some CU7 people who reported and interacted on photometric problems?
\author{
% 1st group: main first 2 authors of the paper
B.~Holl\inst{\ref{inst1},\ref{inst4}}\fnmsep\thanks{Corresponding author: B. Holl
(\href{mailto:berry.holl@unige.ch}{\tt berry.holl@unige.ch})}, %et all
M.~Audard\inst{\ref{inst1},\ref{inst4}},
%2nd group: DPCG, as they otherwise have zero visibility in any other (DR2) papers so far
K.~Nienartowicz\inst{\ref{inst3}}, 
G.~Jevardat~de~Fombelle\inst{\ref{inst3}}, 
O.~Marchal\inst{\ref{inst4},\ref{inst25}}, 
%3rd group: management (part that has not been included yet)
N.~Mowlavi\inst{\ref{inst1},\ref{inst4}}, 
%4rd group (alphabetical): wp leaders all that were run 
G.~Clementini\inst{\ref{inst22}}, % SOS CEP&RRL
J.~De~Ridder\inst{\ref{inst6}}, % classification nTransits:20+
D.W.~Evans\inst{\ref{inst2}}, % CU7 deputy
L.P.~Guy\inst{\ref{inst4},\ref{inst28}}, % added new affiliation, responsible for communication with many modules
A.C.~Lanzafame\inst{\ref{inst7},\ref{inst8}}, % solar-like rotation modulation
T.~Lebzelter\inst{\ref{inst21}}, % long period variables
L.~Rimoldini\inst{\ref{inst4}}, % classification nTransits:2+
M.~Roelens\inst{\ref{inst1},\ref{inst4}}, % short timescale
S.~Zucker\inst{\ref{inst19}}, % TODO: include in RUN list: was active so suggest yes
%5th group (alphabetical): most active DR2 variability contributors
J.~Charnas\inst{\ref{inst4}},
E.~Distefano\inst{\ref{inst8}},
A.~Garofalo\inst{\ref{inst43},\ref{inst22}},
S.~Leccia\inst{\ref{inst12}},
I.~Lecoeur-Taibi\inst{\ref{inst4}},
M.~Lopez\inst{\ref{inst10}}, 
R.~Molinaro\inst{\ref{inst22}}, 
T.~Muraveva\inst{\ref{inst22}},
A.~Panahi\inst{\ref{int19b}},
S.~Regibo\inst{\ref{inst6}},
V.~Ripepi\inst{\ref{inst12}},
L.M.~Sarro\inst{\ref{inst9}},
%6th group (alphabetical): others with low CU7 DR2 activity and including other CU's DR2 activities that helped us
C.~Aerts\inst{\ref{inst6}},
R.I.~Anderson\inst{\ref{inst30}}, % CHECK also Geneva?
F.~Barblan\inst{\ref{inst1}},
S.~Blanco-Cuaresma\inst{\ref{inst1},\ref{inst44},\ref{inst45}},  % updated references
G.~Busso\inst{\ref{inst2}}, % include: asked Dafydd
J.~Cuypers\inst{\ref{inst5}\dag}, % his family agreed
F.~De Angeli\inst{\ref{inst2}}, %  include: asked Dafydd
F.~Glass\inst{\ref{inst1}}, % TODO Check reference OK 
M.~Grenon\inst{\ref{inst1}}, % include!
A.~Juh\'{a}sz\inst{\ref{inst11},\ref{inst27}},
A.~Kochoska\inst{\ref{inst16},\ref{inst50}},
P.~Koubsky\inst{\ref{inst15}}, % yes
A.F.~Lanza\inst{\ref{inst8}},
D.~Lorenz\inst{\ref{inst21}},
M.~Marconi\inst{\ref{inst12}},
G.~Marschalko\inst{\ref{inst11}}, 
T.~Mazeh\inst{\ref{int19b}},
S.~Messina\inst{\ref{inst8}},
F.~Mignard\inst{\ref{inst14}},
A.~Moitinho\inst{\ref{inst18}},	
L.~Moln\'{a}r\inst{\ref{inst42}},
S.~Morgenthaler\inst{\ref{inst20}},
I.~Musella\inst{\ref{inst12}},
C.~Ordenovic\inst{\ref{inst14}},
D.~Ord\'o\~nez\inst{\ref{inst4}}, 
I.~Pagano\inst{\ref{inst8}},
L.~Palaversa\inst{\ref{inst2}}, %  include: asked Dafydd
M.~Pawlak\inst{\ref{inst40},\ref{inst41}},
E.~Plachy\inst{\ref{inst42}}, % DPAC address wrong, says Observatoire de Genève!!! 
A.~Pr\v{s}a\inst{\ref{inst16}}, 
M.~Riello\inst{\ref{inst2}}, 
M.~S\"{u}veges\inst{\ref{inst29}}, 
L.~Szabados\inst{\ref{inst11}},
E.~Szegedi-Elek\inst{\ref{inst42}},
V.~Votruba\inst{\ref{inst15}},
%7th group: team leader
L.~Eyer\inst{\ref{inst1},\ref{inst4}}
% NOT INCLUDED:
% E.~Poretti\inst{\ref{inst26}}, % indicated NO by sending us mail
%Lukasz Wyrzykowski % NO
%%B.~Miranda\inst{\ref{inst18}}, % NO
%%A.~Jan\inst{\ref{inst4}},          % NO
%%G.~Sadowski\inst{\ref{inst17}}, NO
%%M.~Schultheis\inst{\ref{inst14}} NO
%P.~Dubath\inst{\ref{inst4}},   % asked him: NO
%M.~Beck\inst{\ref{inst1}},  % asked LE: No
%F.~van Leeuwen\inst{\ref{inst2}}, %  NOT: asked Dafydd
%B.~Tingley\inst{\ref{inst23}},  % NO
%J.J.~Aguado\inst{\ref{inst9}}, -> NO Luis told us
%J.~Fuchs\inst{\ref{inst15}}, % NO
%M.I.~Ruiz-Fuertes\inst{\ref{inst4}}, % NO
%H.E.~Delgado\inst{\ref{inst9}}, NO
%Y.~Dzigan\inst{},NO
%R.~Hudec\inst{\ref{inst15}}, NO
%A.~Jonckheere\inst{\ref{inst5}}, NO
%P.~Klagyivik\inst{\ref{inst11}}, NO
%A.~Kutka\inst{\ref{inst15}}, NO
%M.~Moniez\inst{\ref{inst24}}, NO
%J.-M.~Nicoletti\inst{\ref{inst20}}, NO
%P.~Park\inst{\ref{inst1}}, NO
%E.~Van~Hemelryck\inst{\ref{inst5}}, NO
%M.~Varadi\inst{\ref{inst11}}, % NO
%
} % TODO remove those not used
\authorrunning{Holl et al.}
\institute{Department of Astronomy, University of Geneva, Ch. des Maillettes 51, CH-1290 Versoix, Switzerland\label{inst1}%\\
%\email{Berry.Holl@unige.ch}
%
\and 
Department of Astronomy, University of Geneva, Ch. d'Ecogia 16, CH-1290 Versoix, Switzerland\label{inst4}
*
\and 
SixSq, Rue du Bois-du-Lan 8, CH-1217 Geneva, Switzerland\label{inst3}
\and
GEPI, Observatoire de Paris, Universit{\'e} PSL, CNRS,  5 Place Jules Janssen, 92190 Meudon, France \label{inst25} % checked withOlivier 
%
\and
INAF Osservatorio di Astrofisica e Scienza dello Spazio di Bologna, Via Gobetti 93/3, I - 40129 Bologna, Italy\label{inst22}
%OLD: INAF - Osservatorio Astronomico di Bologna, Via Ranzani n. 1, 40127 Bologna, Italy\label{inst22}
%
\and
Institute of Astronomy, KU Leuven, Celestijnenlaan 200D, 3001 Leuven, Belgium\label{inst6}
%
\and
Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\label{inst2} % CU5
%
\and
Large Synoptic Survey Telescope, 950 N. Cherry Avenue, Tucson, AZ 85719, USA\label{inst28} % Leanne Guy
%
\and
Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Sezione Astrofisica, Via S. Sofia 78, I-95123 Catania, Italy\label{inst7} 
%
\and
INAF-Osservatorio Astrofisico di Catania, Via S. Sofia 78, I-95123 Catania, Italy\label{inst8}
%
\and
University of Vienna, Department of Astrophysics, Tuerkenschanz\-strasse 17, A1180 Vienna, Austria\label{inst21}
%
\and
Department of Geosciences, Tel Aviv University, Tel Aviv 6997801, Israel\label{inst19}
%
\and 
Dipartimento di Fisica e Astronomia, Universit\`{a} di Bologna, Via Piero Gobetti 93/2, 40129 Bologna, Italy \label{inst43} % note: not same as inst22!
%
\and
INAF-Osservatorio Astronomico di Capodimonte, Via Moiariello 16, 80131, Napoli, Italy\label{inst12}
%
\and
Departamento de Astrof\'isica, Centro de Astrobiolog\'ia (INTA-CSIC), PO Box 78, E-28691 Villanueva de la Ca\~nada, Spain\label{inst10}
%
\and
School of Physics and Astronomy, Tel Aviv University, Tel Aviv 6997801, Israel\label{int19b}
%
\and
Dpto. Inteligencia Artificial, UNED, c/ Juan del Rosal 16, 28040 Madrid, Spain\label{inst9} 
%
\and 
European Southern Observatory, Karl- Schwarzschild-Str. 2, D-85748 Garching b. M\"{u}nchen, Germany\label{inst30} % Richard Anderson
%
\and 
Laboratoire d'astrophysique de Bordeaux, Univ. Bordeaux, CNRS, B18N, all{\'e}e Geoffroy Saint-Hilaire, 33615 Pessac, France \label{inst44}
%
\and 
Harvard-Smithsonian Center for Astrophysics, 60 Garden Street, Cambridge, MA 02138, USA\label{inst45}
%
\and
Royal Observatory of Belgium, Ringlaan 3, B-1180 Brussels, Belgium\label{inst5}
%
\and
Konkoly Observatory, Research Centre for Astronomy \& Earth   Sciences, Hungarian Academy of Sciences, H-1121 Budapest, Konkoly Thege Mikl\'os \'ut  15-17, Hungary\label{inst11}
%
\and 
E\"otv\"os Lor\'and University, Egyetem t\'er 1-3, H-1053 Budapest, Hungary \label{inst27}% provided by LR for Aron Juhász
%
\and
Villanova University, Department of Astrophysics and Planetary Science, 800 Lancaster Ave, Villanova PA 19085, USA \label{inst16}
%
\and
A. Kochoska Faculty of Mathematics and Physics, University of Ljubljana, Jadranska ulica 19,
1000 Ljubljana, Slovenia \label{inst50}
%
\and
Academy of Sciences of the Czech Republic, Fricova 298, 25165 Ondrejov, Czech Republic\label{inst15}
%
\and
Universit\'e C{\^o}te d'Azur, Observatoire de la C{\^o}te d'Azur, CNRS, Laboratoire Lagrange, Bd de l'Observatoire, CS 34229, 06304 Nice cedex 4, France \label{inst14}
%
\and
FCUL, Campo Grande, Edif. C8, 1749-016 Lisboa, Portugal\label{inst18}
%
\and
Konkoly Observatory, Research Centre for Astronomy and Earth Sciences, Hungarian Academy of Sciences, Konkoly Thege Mikl\'{o}s \'{u}t 15-17, 1121 Budapest, Hungary \label{inst42}
%
\and
EPFL SB MATHAA STAP, MA B1 473 (BÃ¢timent MA), Station 8, CH-1015 Lausanne, Switzerland\label{inst20}
%
\and
Warsaw University Observatory, Al. Ujazdowskie 4, 00-478 Warszawa, Poland \label{inst40} % M. Pawlak
\and
Institute of Theoretical Physics, Faculty of Mathematics and Physics, Charles University in Prague, Czech Republic \label{inst41} % M. Pawlak
%
%\and 
%INAF - Osservatorio Astronomico di Brera, Via E. Bianchi 46, I-23807 Merate, Italy \label{inst26} % provided by LR for Ennio Poretti
%
\and
Max Planck Institute for Astronomy, K\"{o}nigstuhl 17, 69117 Heidelberg, Germany\label{inst29} % Maria
%
%\and
%Department of Physics and Astronomy, Johns Hopkins University, 3701 San Martin Dr, Baltimore, MD 21218, USA\label{inst13}
%
%\and
%Institut d'Astronomie et d'Astrophysique (IAA), UniversitÃ© Libre de Bruxelles (ULB), CP 226, Boulevard du Triomphe, B-1050 Brussels, %Belgium\label{inst17}
%
%\and
%Stellar Astrophysics Centre, Aarhus University, Department of Physics and Astronomy, 120 Ny Munkegade, Building 1520, DK-8000 Aarhus C, Denmark\label{inst23}
%
%\and
%Laboratoire de l'AccÃ©lÃ©rateur LinÃ©aire UniversitÃ© Paris-Sud, BÃ¢timent 200,
%91898 Orsay, France\label{inst24}
}

% Other references if needded
%\affil[UNIGE-ECO]{Department of Astronomy, University of Geneva, Chemin d'Ecogia 16, CH-1290 Versoix, Switzerland}
%\affil[UNIGE]{Department of Astronomy, University of Geneva, Chemin des Maillettes 51, CH-1290 Versoix, Switzerland}
%\affil[UCAM]{Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, United Kingdom}
%\affil[SIXSQ]{SixSq, Rue du Bois-du-Lan 8, CH-1217 Meyrin, Switzerland}
%\affil[OAB]{INAF - Osservatorio Astronomico di Bologna, Via Gobetti 93/3, I-40129 Bologna, Italy}
%\affil[OAC]{INAF - Osservatorio Astronomico di Capodimonte, Via Moiariello 16, I-80131 Napoli, Italy}
%\affil[UB]{Department of Physics and Astronomy, University of Bologna, Via Gobetti 93/2, I-40129 Bologna, Italy }
%\affil[OB]{INAF - Osservatorio Astronomico di Brera, Via E. Bianchi 46, I-23807 Merate, Italy}
%\affil[KO]{Konkoly Observatory, Research Centre for Astronomy \& Earth Sciences, Hungarian Academy of Sciences, Konkoly Thege Mikl\'os \'ut 15-17, H-1121 Budapest, Hungary}
%\affil[EU]{E\"otv\"os Lor\'and University, Egyetem t\'er 1-3, H-1053 Budapest, Hungary}
%\affil[KU]{Institute of Astronomy, KU Leuven, Celestijnenlaan 200D, B-3001 Leuven, Belgium}
%\affil[UNED]{Departamento Inteligencia Artificial, UNED, Calle Juan del Rosal 16, E-28040 Madrid, Spain}
%\affil[CSIC]{Departamento de Astrof\'isica, Centro de Astrobiolog\'ia (INTA-CSIC), PO Box 78, E-28691 Villanueva de la Ca\~nada, Spain}

==> figures/Sec_Acknowledgements.tex <==
\begin{acknowledgements}
% TODO add some words concerning Jan Cuypers 
%This work has made use of data from the ESA space mission \textit{Gaia}, processed by the \textit{Gaia} Data Processing and Analysis Consortium (DPAC).
%Funding for the DPAC has been provided by national institutions, some of which participate in the \textit{Gaia} Multilateral Agreement, 
%which include, 
%for Switzerland, the Swiss State Secretariat for Education, Research and Innovation through the ESA Prodex program, the ``Mesures d'accompagnement'', the ``Activit\'{e}s Nationales Compl\'{e}mentaires'', the Swiss National Science Foundation, and the Early Postdoc.Mobility fellowship.\\
%BH has been supported by the ESA Prodex program and currently though the Swiss  ``Activit\'{e}s Nationales Compl\'{e}mentaires''. %, the Swiss National Science Foundation
LL is supported by the Swedish National Space Board.
%\TODO{[TODO: Lennart, Damien and Manuela, please add here (or provide me) with the relevant acknowledgements]}
\EDIT{We would like to thank the referee Alessandro Sozzetti for his detailed remarks and suggestions that much improved the quality and relevance of this paper. Thanks also to Lorenzo Rimoldini, Jeff Andrews, and Danley Hsu for helpful feedback on specific aspects of this paper during its preparation. Thanks to David Katz for discussion on the per-FoV radial velocity error model, and thanks to Laurent Eyer [and Dafydd Wyn Evans if I discuss with him] for their help in the derivation of the photometric per-FoV error model.
%\TODO{Add thanks to those who provided feedback.}
%We acknowledge Mark Taylor for the astronomy-oriented data handling and visualization software TOPCAT
%\citep{2005ASPC..347...29T} used for a few figures in this paper. %We thank ... for valuable feedback during the preparation of this paper. 
This work has made use of data from the European Space Agency (ESA) mission
{\it Gaia} (\url{https://www.cosmos.esa.int/gaia}), processed by the {\it Gaia}
Data Processing and Analysis Consortium (DPAC,
\url{https://www.cosmos.esa.int/web/gaia/dpac/consortium}). Funding for the DPAC
has been provided by national institutions, in particular the institutions
participating in the {\it Gaia} Multilateral Agreement.
}
\end{acknowledgements}


==> figures/Sec_Appendices.tex <==
%\subsection{\gaia detection sensitivity as function of orbit params\label{sec:gaiaResponse}} 
%The \gaia  response function depends on the time sampling (Sect.~\ref{sec:gaiaTs}) and astrometric error model (Sect.~\ref{sec:gaiaError}). Provided these two, we can construct the detection response as function of companion orbital parameters (Sect.~\ref{sec:gaiaResponseComp}).

% Appendix~A
%\subsubsection{\gaia astrometric signal simulation\label{sec:gaiaSim}} 
\section{\gaia time series\label{sec:gaiaTs}} 
We use AGISLab \citep{Holl:2012fk} to simulate the actual Gaia scanning law for the 5-yr nominal and 10-yr extended mission\footnote{From 
%tMin = 2014.7337440109513 ISO: 2014-09-26T00:00:00.000 (TCB) % start of NSL
%t5year:=2019.7337440109513 ISO: 2019-09-26T06:00:00.000 (TCB) % 5 year after NSL start
%t10year= 2024.7337440109513 ISO: 2024-09-25T12:00:00.000 (TCB) % 10 year after NSL start
Julian year 2014.734 (2014-09-26, start of Nominal Scanning Law phase)  
to 2019.734 (2019-09-26) for the nominal 5-year mission, and up to 2024.734 (2024-09-25)  for the 10-yr extension.
}. 
We have used a uniformly distributed grid of 784 sky positions, these %\TODO{XXX} deg$^2$ each 
being the bin centres of a level 3 HEALPix map \citep{Gorski:2005qy}. 
A histogram of the number of field-of-view observation of all the simulated time series is shown in Fig.~\ref{fig:FovNumObs}.
The simulated Besan\c con star positions are then mapped to the time series of the nearest neighbour on this grid. 
For each simulated source, each observations of a time series has a 10\% chance to be randomly removed in order to account for the expected mission dead-time.

\begin{figure}[b]
 \includegraphics[width=0.49\textwidth]{figures/SimNumFov.pdf} 
\caption{Distribution of the simulated number of field-of-view (FoV) observations of the 196 sky positions used in this study for a 5- and 10-yr \gaia mission (bin size: 10). For radial velocity measurements the number of FoV observations is reduced by a factor of 0.57 (4/7, see Sect.~\ref{sec:gaiaDetectMethodTransit}).
}
\label{fig:FovNumObs}
\end{figure} 



% Appendix~B
\section{\gaia astrometric FoV error model\label{sec:gaiaError}} 

\begin{figure}[hbt]
 \includegraphics[width=0.49\textwidth]{figures/accLaws.pdf} 
\caption{Adopted \EDIT{astrometric} \gaia per-FoV precision model compared based on the expected \gaia precision derived from DR2 data, and compared with the  \cite{2014ApJ...797...14P} error model.
}
\label{fig:FovAccLaw}
\end{figure} 
With the \gaia mission and its calibration improvements still in progress, we adopt the same astrometric observation error model parameterisation described in Sect.~2.1 of \cite{2014ApJ...797...14P}.
%, which was based on the estimated end-of-mission performance of \gaia. 
This error model provides the per-field-of-view astrometric centroiding error 
$\sigma_{\textrm{fov,astro}}$ ($\mu$as) as a function of the host-star $G$-band magnitude: 
\begin{eqnarray} 
z &=& 10^{0.4(\textrm{max}[G,12]-15)} \nonumber \\
\sigma_\eta&=&( c_1\ z + c_2 \ z^2)^{0.5} \nonumber \\
\sigma_{\textrm{fov,\,astro}} &=& \left( \frac{ \sigma^2_\eta }{9} + \sigma^2_{\textrm{att}} +  \sigma^2_{\textrm{cal}}  \right)^{0.5}  \textrm{[$\mu$as]} \label{eq:fovPrecision}
\end{eqnarray}
\begin{eqnarray} 
 &\text{with}&  c_1= 53\,000 \text{ and } c_2= 310 \text{ in \cite{2014ApJ...797...14P}} \nonumber \\
 &\text{and}&  c_1= 49\,000 \text{ and } c_2= 1700 \text{ in this work (DR2 fit).} \nonumber 
\end{eqnarray}
Note that for bright stars with $G<12$ the observation times are reduced by CCD `gating' to avoid signal saturation, causing a more or less constant measurement precision for these stars. In this error model it is assumed to be strictly constant at a level of $\sigma_{\textrm{fov}}=  34 \ \mu$as per field-of-view when adopting a value of 20 $\mu$as per field-of-view transit for both  $\sigma^2_{\textrm{att}}$ and $\sigma^2_{\textrm{cal}}$ \citep{Risquez:2013aa, Lindegren:2012aa}, corresponding to a combined attitude and calibration noise level of 
%%sqrt(9)*sqrt(2)*20 = 85 uas
85 $\mu$as  per CCD.  The current DR2 per-CCD astrometric centroiding precision shown in Fig.~9 of \cite{Lindegren:2018aa} illustrates that the current systematic noise level is about 250~$\mu$as per CCD. We here make the realistic assumption that this noise level will reduce by a factor of three for the final astrometric data release due to improved calibration models. 

The free parameters $c_1$ and $c_2$ of the \cite{2014ApJ...797...14P} error model of Eq.~\ref{eq:fovPrecision} were adjusted to fit the pre-launch prediction of the end-of-mission astrometric performance. We can revise this fit based on the latest estimates from DR2, as shown in Fig.~\ref{fig:FovAccLaw}. The circles are DR2 median per-CCD formal uncertainties from Fig. 9 in \cite{Lindegren:2018aa}, converted to per-FoV estimates by dividing them by the square root of the 9 per-FoV CCDs, and increased by 10\% to match the actual robust scatter estimate observed, particularly for the fainter sources,  in the Astrometric Global Iterative Solution \citep[AGIS, ][]{Lindegren:2012aa, 2011ExA....31..215O, 2010ASPC..434..309L}. It is not expected that the calibration precision will further improve for $G>13$ where it is photon-limited. 

The \cite{2014ApJ...797...14P} and our DR2 derived error models agree within a few percent up to $G\sim17$, and start to deviate thereafter (8\% at $G=17.5$, 13\% at $G=18$, etc...), mainly due to the increased stray-light component in the real mission data. The \cite{2014ApJ...797...14P} predicted planet detections were basically brighter than $G=17$ and hence their conclusions would be unchanged based on this latest model. Our results extend to $G=17.5$, and hence this new error model will reduce the number of detections towards the faint end.

% MACP: I suggest that this is not relevant here, and so delete
\EDIT{This error model has already been been used in \cite{2019ApJ...886...68A} through means of private communication.}

% formal uncertainty, compared to a fit to the current DR2 data and assuming the aforementioned $85\ \mu$as/CCD noise floor, which limits the per-FoV precision to about $34\ \mu$as. Note that for $G>13$ we do not expect the calibration precision to improve further as it is dominantly photon-limited. The error models agree within a few percent up to $G\sim17$, and start to deviate thereafter (10\% at G=17.5), mainly due to the increased stray-light component in the real mission data. As we only used  Besan\c con data with G<17.5 we stick with the convenient \cite{2014ApJ...797...14P} model. \TODO{[or should we give and use to the new derived function?]}.

%The precision at the faint end is $966.5 \ \mu$as for G=20 mag, see Table~2 of \cite{2014ApJ...797...14P} for details.


% Appendix~C
\section{\EDIT{\gaia radial velocity FoV error model}\label{sec:gaiaErrorRv}} 

\begin{figure}[hbt]
 \includegraphics[width=0.49\textwidth]{figures/FINAL_RvPrecisionFitWith0p11noiseFloor.pdf} 
\caption{\EDIT{Adopted radial velocity \gaia per-FoV precision model valid for $G_{\text{RVS}}<12$, derived from \gaia DR2 radial velocity data.}
}
\label{fig:FovAccLawPhot}
\end{figure} 
\EDIT{To compute the detectability of BD companions using the \gaia RVS derived radial velocity measurements (Sect.~\ref{sec:gaiaDetectMethodRv}) we need an end-of mission estimate of the per-FoV precision of the radial velocity measurements. Due to changes from the pre-launch conditions \citep[e.g.\ the stray-light issue discussed by the][]{2016A&A...595A...2G} we estimated the expected end-of-mission performance from the currently available data, i.e., Fig.~18 of \cite{2019A&A...622A.205K}. We take the data points for the interval of [7,11] transits which have a mean at $N=8$, and using their Eq.~1 we fit a fifth degree polynomial model $P(G_{\text{RVS}})$ to the `formal' per-FoV transit uncertainty $\sigma_{\text{V}_\text{R}}$
\begin{equation}
\epsilon_{\text{V}_\text{R}} = \left[ \left( \sqrt{ \frac{\pi}{2\ N}} P(G_{\text{RVS}}) + 0.11^2 \right) \right] \ \ \text{with} \ \ P(G_{\text{RVS}}) \simeq \sigma_{\text{V}_\text{R}}	\ ,
\end{equation}
with the polynomial model
\begin{eqnarray}
P(G_{\text{RVS}}) &=& -1.430 + 2.944 x  -1.3084 x^2 + 0.25102 x^3\nonumber  \\
&&  -0.021959 x^4 + 0.00072645x^5 \\
\text{with} \ \ x&=& \text{max}\left(2.26, G_{\text{RVS}}\right) \nonumber
\end{eqnarray}
For the adopted per-FoV precision we include a 0.11\,km\,s$^{-1}$ noise floor, which is the current best estimate for the end-of mission precision (David Katz, private communication), resulting in
\begin{equation}
\sigma_{\text{fov,\,RV}} =  \sqrt{ P^2(G_{\text{RVS}}) + 0.11^2 } \ \ \textrm{[km\,s$^{-1}$]}	\ .
\end{equation}
}




% Appendix~D
\section{\EDIT{\gaia photometric FoV error model}\label{sec:gaiaErrorPhot}} 

\begin{figure}[hbt]
 \includegraphics[width=0.49\textwidth]{figures/edr3_vs_dr2.png} 
\caption{\EDIT{Adopted photometric \gaia G-band per-FoV precision model compared based on the approximate \gaia precision derived from EDR3 data.}
}
\label{fig:FovAccLawPhot}
\end{figure} 
\EDIT{To compute the detectability of photometric brown dwarfs transits (Sect.~\ref{sec:gaiaDetectMethodTransit}) we require an end-of mission estimate of the per-FoV precision of the $G$-band photometry. As for the radial velocity precision, we have replaced the pre-launch estimates with those from currently available data. In Fig~\ref{fig:FovAccLawPhot} we estimate the per-FoV $G$-band photometric precision (blue solid lines) from the published uncertainties on the mean, for both DR2\footnote{\EDIT{This traced in a rough way the orange mode-line of the distribution in Fig.~9 of \cite{2018A&A...616A...4E}, and is rescaled to represent the corresponding precision per FoV (in absence of any noise floor). Note that \textit{meanCcdPerFov} represents the number: 8.857 = (6/7*9+1/7*8), i.e., the focal plane has 7 rows of CCDs of which one has 8 CCDs and the other have 9 CCDs that are used to derive G-band photometry.}} (black line) and EDR3\footnote{\EDIT{We query a random sample of 1M EDR3 sources with a minimum of 150 CCD observations (\texttt{phot\_g\_n\_obs}) and directly scale them to the (noise-floor free) per-FoV precision in magnitude: \texttt{fov\_uncertainty\_mag= 1.0857/sqrt((6/7*9+1/7*8))*phot\_g\_mean\_flux\_error *sqrt(phot\_g\_n\_obs)/ phot\_g\_mean\_flux}.}} (scatter data). From this we see that above $G>16.5$ the improvement in EDR3 is relatively small. From this observation, and the fact that it extends down to about $G=13.5$ along a rather straight exponential line, we will assume that the EDR3 mode-line reached the photon limited precision and will no further improve in future releases. For the bright range the gating complicates the calibrations, and it is clear that this has substantially improved in EDR3, and should continue to improve in the coming releases. Therefore we adopted a simple noise floor of $\sigma_\text{FoV,\,G}=10^{-3}$\,mag\footnote{\EDIT{This coincides with the pre-launch estimate of 1\,mmag adopted by \cite{2012ApJ...753L...1D}. At that time it was assumed this floor would extend to $G=14$ or beyond, such that their predicted transit counts fainter than 14~mag should be considered as somewhat optimistic.}}, which effectively extends up to $G\simeq13.5$. For $G>13.5$ we fit a second-order polynomial to the mode of the EDR3 data, resulting in our adopted model, illustrated by the blue line
\begin{eqnarray}
    \sigma_\textrm{fov,G} &=& 10^{\text{max}\left[-3, -3.56 \ -0.0857\, x \ + \ 0.00938\, x^2 \right]} \ \ \textrm{[mag]} \\
 \text{with }   x &=& G-0.15 \nonumber 	\ .
\end{eqnarray}
}

%\section{Tabulated \gaia detection limits of unseen companions\label{sec:responseFunctionResults}} 
%Besides the \gaia detection sensitivity in the BD mass range described in Sect.~\ref{sec:gaiaResponseComp}, we provide in the online material a table with the detection limits for a much larger range of (unseen) companion masses from $1M_{\text{J}}$ to $100M_{\odot}$, with eccentricities between 0~and~0.95, for a host star mass range $0.36-2.3M_{\odot}$. A preview of these data is provide in Table~\ref{tab:gaiaResponse}. 

%\begin{table*}[h]
%\caption{Tabulated sensitivity function \TODO{[will add first few rows and column explanation in next revision]}
%}. 
%\label{tab:gaiaResponse}     
%\centering                        
%\begin{tabular}{l r r | c c c c c}        
%\hline\hline      
%\multicolumn{3}{c|}{Host star ($A_v=0$)}  & unseen companion mass & period & ecc %&  mission duration &  distance [pc]\\
%type & G$_{\hbox{abs}}$   & M$_{\odot}$      &  \mjup or \msol                  &                    day          &       &    yr   & for $\Delta \chi^2$ threshold: \\
%\hline 
%F0V & 3.0 & 1.7 &  \{1~M$_{\rm{J}}$  -- 100~M$_{\odot}$\}\tablefootmark{a} 
%				 &  \{$1-10^5$\}\tablefootmark{b} 
%				 &  \{$0-0.95$\}\tablefootmark{c}
%				 & \{$5-10$\}
%				 & \{$>30$, $>50$, $>100$\} \\
%G2V & 5.0 & 1.0 & \\
%K5V & 7.4 &0.69 & \\
%\hline                                 


%\hline                                             %inserts single line
%\end{tabular}
%\tablefoot{\newline
 %       \tablefoottext{a}{$\Delta \log{\text{M}}$=0.5: 1~\mjup,  3.16~\mjup, 10~\mjup, 31.6~\mjup, 100~\mjup, 320~\mjup, 1~\msol, 3.16~\msol, 10~\msol, 31.6~\msol, 100~\msol.}\newline
 %       \tablefoottext{b}{$\Delta \log{\text{P}}$=0.2: 1~d, 1.6~d, 2.5~d, 4.0~d, 6.3~d, 10~d, 16~d, $\dots$ , $10^5$~d}\newline
 %       \tablefoottext{c}{eccentricities: 0, 0.3, 0.6, 0.8, 0.9, 0.95}
%}
%\end{table*}





%
%
%hostStarMass_msol,bd_mjup,massRatio,gMag,ecc,semiMajAxis_au,distance_pc,parallax_mas,semimajorAxis_mas,period_day,tMax,nObsMean,nObsMin,nObsMax,lambdaMean,lambdaFracGt23,lambdaFracGt43,lambdaFracGt93
%
%
%\begin{sidewaystable*}
%{\footnotesize\begin{minipage}[t][180mm]{\textwidth}
%\caption{Statistical parameters for the SOS types published in DR2. The 1\%, 50\% (median), and 99\% percentile
%    are provided for each type.\label{tbl:tsrStatSOS}}
%\begin{tabular}{lr@{\,\,\,\,}r@{\,\,\,\,}rr@{\,\,\,\,}r@{\,\,\,\,}rr@{\,\,\,\,}r@{\,\,\,\,}rr@{\,\,\,\,}r@{\,\,\,\,}rr@{\,\,\,\,}r@{\,\,\,\,}r}
%\hline\hline
%\relax\\[-1.7ex]
%hostStarMassl,bd,,g, ecc, semiMajAxis12, distance, parallax, semimajorAxis,period,tMax,nObsMean,nObsMin,nObsMax, lambdaMean, lambdaFracGt23,lambdaFracGt43,lambdaFracGt93 \\
%$M_\text{sol}$msol,$M_\text{J$, ,mag, ,au,pc,mas,mas,day,yr,,,,,,, \\
%
%
%$G$ band  & \multicolumn{3}{c@{}}{Cepheids} & \multicolumn{3}{c@{}}{RR Lyrae stars} & \multicolumn{3}{c@{}}{Long-period var.}
%        & \multicolumn{3}{c@{}}{Rot.~Modulation} & \multicolumn{3}{c@{}}{Short timesc.}\\
%\cmidrule(l){2-4}
%\cmidrule(l){5-7}
%\cmidrule(l){8-10}
%\cmidrule(l){11-13}
%\cmidrule(l){14-16}
%%Filtered number of FoV transits & $15$ & $28$ & $118$ & $13$ & $27$ & $81$ & $12$ & $27$ & $69$ & $24$ & $43$ & $88$ & $19$ & $32$ & $69$ \\ 
%%Time duration (d) & $514.00$ & $627.70$ & $667.48$ & $430.10$ & $593.78$ & $657.13$ & $427.22$ & $591.78$ & $638.78$ & $481.77$ & $580.21$ & $651.04$ & $475.32$ & $587.09$ & $642.99$ \\ 
%\hline
%
%
%\end{tabular}
%\tablefoot{
%\tablefoottext{a}{For RR Lyrae stars, the percentiles for $G_{\rm BP}$ and $G_{\rm RP}$ were computed for a number of FoV transits $>1$,
%    although there are stars with $0$ or $1$ transit remaining in the band after our cleaning. For the skewness and kurtosis, we
%    included only RR Lyrae stars with $>2$ and $>3$ transits, respectively.}
%}
%\vfill
%\end{minipage}
%}\end{sidewaystable*}
%
%


% ---------------------------


% Appendix~E
\section{Cumulative density functions\label{sec:cdfMass}} 

To generate $(M_{\mathrm{BD}})$ from a uniform distributed random number $U\sim U([0,1])$
we use the inverse cumulative density function. This is the inverse CDF of Eq.~\ref{eq:massDCF}:
\begin{equation}
% CDF_M^{-1}(u)= \frac{- b \pm \sqrt{b^2 -4ad}}{2a} = x \quad \text{ with: } \quad  d= c-u
    {\rm CDF}_\text{M}^{-1}(u)=\begin{cases}
    \frac{- b + \sqrt{b^2 -4a(c-u)}}{2a}, & \text{$\ \ \ \ \ 0\leq u <0.49$} \\
   (u-c)/b, & \text{$0.49\leq u<0.51$}\\
    \frac{- b + \sqrt{b^2 -4a(c-u)}}{2a}, & \text{$0.51 \leq u \leq 1$}
    \label{eq:invMassDCF}
  \end{cases}
\end{equation}
where the coefficients correspond to those presented in Eq.~\ref{eq:massDCF}.
Using the same technique the random sampling of the period and eccentricity distribution were performed, using the inverse functions of the CDF formulae given in Figs.~\ref{fig:cdfHistPeriodFit} and \ref{fig:eccDist}.



% Appendix~F
\section{Besan\c con model data for $G>10.5$ \label{appendix:besancon}}

\EDIT{To simulate the vast majority of the host star distribution we used the  latest 2016\footnote{\url{http://modele2016.obs-besancon.fr/}}  Besan\c con model}, which has various improvements over the model of 2013, 
%like a no longer constant 
including a variable star formation rate over the thin disk life time \citep{2014A&A...564A.102C}.
%The only configurable parameter, t
The extinction distribution was set to the suggested  \cite{2006A&A...453..635M} model for $100\degr < l < 100 \degr $ and $-10\degr < b < 10\degr$, and diffuse extinction for higher latitudes and longitudes.

% First version, but redone after
%Simulations were run with a sampling of 10\degr steps in Galactic longitude l = 0\degr to 180\degr  \TODO{[is it  symmetric for 180\degr - 360\degr?]} and Galactic latitude b = 0\degr  to 25\degr with a step size of 5\degr, the latitude above 25\degr were sampled with a step size of 18\degr  in Galactic longitude (in range l = 0\degr to 180\degr) and a latitude step size of 6.5\degr from b = 25\degr to 90\degr. 
% extract from selections in analyses.fits+ (of the 1 quadrant BSC simulation):
%_1	All		5049974	100% 		4*5049974 = 20'199'896		
%_2	CL=5	2010816	40% 	CL==5	4*2010816 = 8'043'264		
%_3	CL=4	1124572	22% 	CL==4	4*1124572 = 4'498'288		
%_4	CL=3	1882020	37% 	CL==3	4*1882020 = 7'528'080		
%_5	CL=2	32479	1% 	CL==2	4*32479 = 129'916		
%_6	CL=1	87		0% 	CL==1	4*87 = 348	
%The number of generated sources is:  20\,199\,896 % from 4x quadrant
%which are subdivided in luminosity classes as follows: V=8.0~M (Main Sequence), IV=4.5~M (Subgiants), III=7.5~M (Giants), II=130~K (Bright Giants), and I=0.3K (Supergiants). 


Simulations were generated in bins adjusted for three zones: (1)~the `outer' Galactic northern and southern hemispheres spanning $0\degr \leq l < 360 \degr$ in steps of $36\degr$, and $28\degr < |b|  \leq90\degr$ in steps of $6.2\degr$;
(2) the Galactic `centre' region spanning $-60\degr \leq l \leq 60 \degr$ in steps of $10\degr$, and $-28\degr \leq b  \leq28\degr$ in steps of $3.5\degr$; and (3) the Galactic `disk' region spanning $60\degr < |l| \leq 180 \degr$ in steps of $20\degr$, and $-28\degr \leq b  \leq28\degr$ in steps of $3.5\degr$.
% extract from selections in B_output.fits  (25 GB combined):
%_1	All		130327900	100%
%_2	CL=5	  92863736	71.25%
%_3	CL=4	  37464164	28.75%

The model includes the apparent \gaia $G$-band magnitude. Although the simulated $G$~passband uses the pre-launch transmission curves described in \cite{Jordi:2006aa, Jordi:2010aa}, any differences with the in-flight passband will be negligible for the outcome of this study.
The simulations were limited to spectral types from F0 to K9, and Luminosity class IV~(subgiants) and V (main sequence).  
%\TODO{[Repeat?] because the majority of the host star's lifetime will be spent in these evolutionary stages. [Correct?/Clarify?:] Also, astrometric companion detection around giants might be hindered by spots or other effects that increases the astrometric noise.}  
A limit of $G<17.5$ was adopted based on the low detection-rates beyond this magnitude \EDIT{(see Appendix~\ref{sec:gaiaDetectionLimits})}, and otherwise rather excessive simulation data volume.
% \TODO{[I plan to run extra simulations perhaps up till 18.5 to get the more complete sample]}.



The Besan\c con model output contains generated stars that are sampled uniformly in density for each of the sky-position bins. %, as shown in Fig.~\ref{fig:bscSkydensity}.
The total number of generated sources is: 130\,327\,900 of which 92\,863\,736~(71\%) are main sequence stars, and 37\,464\,164~(29\%) are sub-giants. Fig.~\ref{fig:bscFig1} shows the distribution of stars: on the sky, as function of magnitude, stellar type, and as function of effective temperature versus mass and bolometric magnitude. The bottom panel has some visual guides at $T_{\text{eff}}=7220$\,K and 3940\,K, and $M_{\text{bol}}=2.50$ and 7.59, corresponding to the main sequence F0 and K9 stars\footnote{\label{footnoteMamajek}V2019.3.22 (Eric Mamajek) of \url{http://www.pas.rochester.edu/~emamajek/EEM_dwarf_UBVIJHK_colors_Teff.txt}} \citep{Pecaut:2013aa}.

 \EDIT{
The Besan\c con model we extracted did not contain any stars with $G<10.2$\,mag. For this paper we therefore use \gaia DR2 derived data for $G<10.5$ (Appendix~\ref{appendix:gaiaGt10p5}) and use the Besan\c con data for $G>10.5$.}

\EDIT{
We also require $G_{\text{RVS}}$ to select sources which are assumed to have radial velocity time series (i.e. $G_{\text{RVS}}<12$). 
%This can be derived from the $G$-band magnitude and colour of each system. 
As our Besan\c con data uses the pre-launch \gaia magnitude system \citep{Jordi:2010aa}, we use those relations to compute $G_{\text{RVS}}$ from the $G$-band magnitudes and colours. 
%(12-0.06921061)/0.9361332 -12 = 0.7447
A $G_\text{RVS}=12$ corresponds roughly to $G=12.65$ for our FGK main sequence and sub-giant sample. Applying the exact limit of $G_{\text{RVS}}<12$ on our Besan\c con data with $G>10.5$  results in a sample of 1.7~million stars.}


% Appendix~G
\section{\gaia DR2 derived data for $G<10.5$ \label{appendix:gaiaGt10p5}}
\EDIT{Because the Besan\c con model data did not contain stars brighter than $G<10.2$, we derived the stellar distribution for $G<10.5$ from \gaia DR2 data. For the simulations in this study we need positions, apparent G-band magnitudes, distances, stellar host masses, radii, and $G_{\text{RVS}}$ magnitude estimates. %(the radii are only used for transit probability computations). 
The position \citep{Lindegren:2018aa}, apparent magnitude  \citep{2018A&A...616A...3R,2018A&A...616A...4E}, and estimate of the radius \citep{2018A&A...616A...8A} are available in DR2. 

For about 95\% of DR2 sources the \texttt{parallax\_over\_error>5} (i.e., relative error better than 20\%)
%and in our final sample (discussed below) this is true for all the sources, which 
which means that a simple inverse of the parallax provides a meaningful distance, although it can still be biassed and have a large uncertainty. Since we are mainly interested in the \textit{local} stellar density, we used the bayesian estimated distances with Galactic prior of \cite{2018AJ....156...58B} to derive a meaningful distance estimate for the whole sample\footnote{\texttt{r\_est} from: \url{http://gaia.ari.uni-heidelberg.de/tap.html}}. Distances for our final sample typically deviate from the inverse parallax by less than 1\% (and by a maximum of 8\%).

To make an (initial) selection of main sequence and sub-giants stars we use the main sequence selection of FGK stars in \gaia DR2 described in Section~3.1 of \cite{Hsu_2019}, with their suggested $G_{BP}-G_{RP}$ range of [0.5, 1.7]. We made the following DR2 archive selection:
\texttt{lum\_val < 3*1.75*power(10, 2.62 - 3.74*bp\_rp + 0.962*bp\_rp*bp\_rp)}, where we added the factor~3 to confidently include the increase in luminosity from main sequence to sub-giants phase (which is around 3 for solar-type stars, and more like 1.8 for F-type stars), resulting in a preliminary selection of 204\,433 stars. In the \cite{Hsu_2019} paper the power of 10 was erroneously not mentioned (Danley Hsu, priv.\ comm.). 

Mass estimates were not yet included in DR2. In comparison with the brightest part of the Besan\c con data, masses of the current observable sample can be reasonably well estimated from the absolute magnitude alone, with a dispersion of about $0.2~M_{\odot}$. We fit this relation with a quadratic function for the zero-age main sequence masses of the FGK stars listed in \cite{Pecaut:2013aa}\textsuperscript{\ref{footnoteMamajek}}: $M /M_{\odot} = 2.4571 - 0.41272 G_{{\text{abs}}} + 0.022355 G_{{\text{abs}}}^2$, which correctly follows the core of the distribution of both the main sequence and sub-giants in Besan\c con mass versus $G  -5 \log10( \text{distance [pc]})+5$ (extinction correction does not have a large effect).
Because the most massive stars in our sample (F0) should not exceed $1.6M_{\odot}$, we select only stars with $M<1.6M_{\odot}$. This modifies our initial selection based on the luminosity as a function of $G_{BP}-G_{RP}$ such that the most luminous tip at the blue end gets clipped around a luminosity of $8.5 L_{\odot}$, which is similar to a F0V zero-age main sequence luminosity of $7.8L_{\odot}$, and about 1.8 times less than $4.6L_{\odot}$ for a F3V  zero-age main sequence star \citep{Pecaut:2013aa}\textsuperscript{\ref{footnoteMamajek}}, illustrating that such a cut should roughly retain the relevant sub-giants and not include too many giants. We estimate the absolute magnitude for the \gaia DR2 sources using \texttt{phot\_g\_mean\_mag - 5*log10(r\_est [pc]) + 5}. The extinction \texttt{a\_g\_val} is missing for about 25\% of the sources in our selection and for those who have it, it causes peculiar (non-physical) structures in our HR-diagram, hence we omit any extinction correction.
We then estimate the masses based on this derived absolute magnitude and apply the mass-cut of $M < 1.6 M_{\odot}$ which reduces our \gaia DR2 sample to a final 174\,122 stars with $G<10.5$.

Additionally, we would like to roughly separate the main sequence stars from the sub-giants, as in the Besan\c con data. The Besan\c con data shows that a cut of $R_{\odot}>1.7$ should contain the vast majority of the sub-giants, and below that the vast majority of the main-sequence stars. This makes sense given that this it about the zero-age main-sequence radius of our largest considered stars \citep[F0V-F1V,][]{Pecaut:2013aa}\textsuperscript{\ref{footnoteMamajek}}, Even though this separation is not perfect, the distributions of the Besan\c con and Gaia DR2 selected data sets overlap rather well in the colour-magnitude diagram, and are consistent with their expected location in this diagram. In this way we classify the selected 174\,122 DR2 stars in to 113\,832 (65\%) main sequence stars, and 60\,290 (35\%) sub-giants.

%with the kind of selections one would draw `by hand'.
%when inspecting the \gaia DR2 HR-diagram plotted data (i.e., estimated absolute magnitude versus $G_{BP}-G_{RP}$).


Finally, we need $G_{\text{RVS}}$ to select sources which are assumed to have radial velocity time series (i.e. $G_{\text{RVS}}<12$). Since there is no prescription yet available to convert \gaia DR2 photometry into $G_{\text{RVS}}$, we simply adopt the approximate mode offset of about 0.65\,mag, i.e., $G_{\text{RVS,\,DR2}}= G_{\text{DR2}}+0.65$ to all DR2 stars, irrespective of colour. 
The standard deviation around the mean offset in the Besan\c on model was around 0.11~mag, hence we expect this fixed-value offset approximation to give meaningful approximations to the real $G_{\text{RVS}}$. Needless to say, all selected DR2 stars with $G<10.5$ were thus selected in our sample which were assumed to have radial velocity timeseries, i.e., $G_{\text{RVS}}<12$.

}


%There are some few hundred thousand\footnote{E.g., in the \gaia DR2 archive we find about two hundred thousand stars for the rough selection: $4000<T_\text{eff}<7000$~K with $G<10.2$ and $\varpi>2$~mas.}  
%main sequence and subgiant FGK stars brighter than this limit, for which the detection should be rather complete (see Fig.~\ref{fig:gaiaDetectability}), resulting in a missing sample of perhaps 1000--1500 BD systems (with the 0.6\% BD occurrence rate adopted in Sect.~\ref{sec:bdFractHostStars}) that are not simulated in this paper. Though these targets are extremely interesting for spectroscopic follow-up (see Sect.~\ref{sec:implications}), it will turn out that this is just a marginal number compared the total estimated detectable BDs.
% will not alter our es though the relative number of stars rather low compared to the fainter  We will estimate the missed amount of BDs due to this absent part of the data in Sec.~\ref{sec:missingBrightHost}.








%\section{SN-detection criterion comparison\label{appendix:snCrit}}
%For completeness we also provide the results based on the  more simplistic SN-criterion, and its overlap with the $\Delta \chi^2$ criterion.   Fig.~\ref{fig:snCritComparison} illustrates the differences. For example, for a 5-yr mission the $\Delta \chi^2>30$ seems to correspond roughly to SN\,>\,1.0, while for a 10-yr mission this is somewhere between 0.5--1.0. Similarly, the $\Delta \chi^2>100$ seems to roughly correspond to SN\,>\,2.0 and for a ten-year mission between 1.0--2.0. A more quantitative overview is presented in Table~\ref{tab:simResultsSnCrit}.


%\begin{figure*}[h!]
%  \vspace{0cm}\\
%  \includegraphics[width=0.49\textwidth]{figures/SnVsMag5yrMa14fit.png} 
%    \includegraphics[width=0.49\textwidth]{figures/SnVsMag10yrMa14fit.png} 
%\caption{Comparison of the SN-criterion vs the three different BD detection thresholds: $\Delta~\chi^2 >30$~(38\,000), $\Delta~\chi^2~>50$~(26\,000), and $\Delta~\chi^2 >100$~(16\,000) resulting from the 5-year \gaia simulation with the `Ma\,\&\,Ge' period distribution.}
%\label{fig:snCritComparison}
%\end{figure*} 


%\begin{table*}[t]
%\caption{Number of BDs from simulation based on the SN criterion ($a_*/\sigma_{\text{fov}}$) in comparison to the $\Delta \chi^2$ criterion. %The number of BDs is tabulated. %, with in parentheses their number of host stars having photometric transits in \gaia data together with the mean number of transits. 
%`Ma\,\&\,Ge'  and `D\' iaz' refer to the two period distribution fits in Sect.~\ref{sec:bdPriors} (Fig.~\ref{fig:cdfHistPeriodFit}).
%All numbers are for an assumed BD occurrence rate of $0.6\%$, for which we assume an uncertainty of $\pm 0.3\%$ meaning the numbers could be up to $50\%$ higher or lower (see Sect.~\ref{sec:bdFractHostStars}). %\TODO{[I need to fill in the transit numbers if you think relevant]}
%}. 
%\label{tab:simResultsSnCrit}     
%\centering    
%%\renewcommand{\arraystretch}{1.0}                    
%\begin{tabular}{c c c | r @{\ }l r@{\ } l }          % 
%\hline\hline      
%Mag selection & $a_*/\sigma_{\text{fov}}$ & $\Delta \chi^2$ & \multicolumn{2}{c}{Ma\,\&\,Ge}    & \multicolumn{2}{c}{D\' iaz} \\
%\cline{2-5}    
 %&  & & \multicolumn{2}{c}{Ma\,\&\,Ge }   & \multicolumn{2}{c|}{D\' iaz} & \multicolumn{2}{c}{Ma\,\&\,Ge }   & \multicolumn{2}{c}{D\' iaz}  \\    % table heading
%\hline                                 
%ALL &	>0.5	& ALL 			& 96\,000 &   & 116\,000 &  \\
%ALL &	>1	& ALL 			& 46\,000 &   & 57\,000 &  \\
%ALL &	>2	& ALL			& 20\,000 &   & 24\,000 &  \\
%ALL &	>3	& ALL			& 11\,000 &   & 14\,000 & 	 \\
%ALL &	>6	& ALL 			& 3\,900 &   & 4\,900 &  \\
%\hline
%ALL &	>0.5	& $>30$ 			& 40\,000 &   & 49\,000 &  \\
%ALL &	>1	& $>30$ 			& 38\,000 &   & 46\,000 &  \\
%ALL &	>2	& $>30$ 			& 20\,000 &   & 24\,000 &  \\
%ALL &	>3	& $>30$ 			& 11\,000 &   & 14\,000 &  \\
%ALL &	>6	& $>30$			& 3\,900 &   & 4\,900 &  \\
%\hline
%ALL &	>0.5	& $>50$ 			& 27\,000 &   & 34\,000 &  \\
%ALL &	>1	& $>50$ 			& 27\,000 &   & 34\,000 &  \\
%ALL &	>2	& $>50$ 			& 19\,000 &   & 23\,000 &  \\
%ALL &	>3	& $>50$ 			& 11\,000 &   & 14\,000 &  \\
%ALL &	>6	& $>50$			& 3\,900 &   & 4\,900 &  \\
%\hline
%ALL &	>0.5	&  \ \ $>100$ 		& 17\,000 &   & 21\,000 &  \\
%ALL &	>1	&  \ \ $>100$ 		& 17\,000 &   & 21\,000 &  \\
%ALL &	>2	&  \ \ $>100$ 		& 15\,000 &   & 19\,000 &  \\
%ALL &	>3	&  \ \ $>100$ 		& 11\,000 &   & 14\,000 &  \\
%ALL &	>6	&  \ \ $>100$		&  3\,900 &   & 4\,900 &  \\
%\hline
%$G_{\text{RVS}}<12$ & >0.5 	& ALL 		& 7\,800 &   & 8\,500 &  \\
%$G_{\text{RVS}}<12$ & >1 	& ALL 		& 6\,100 &   & 6\,900 &  \\
%$G_{\text{RVS}}<12$ & >2 	& ALL 		& 4\,300 &   & 5\,000 &  \\
%$G_{\text{RVS}}<12$ & >3	& ALL 		& 3\,200 &   & 3\,900 &  \\
%$G_{\text{RVS}}<12$ & >6 	& ALL 		& 1\,700 &   & 2\,100 &  \\
%\hline
%$G_{\text{RVS}}<12$ &	>0.5	& $>30$ 			& 5\,700 &   & 6\,500 &  \\
%$G_{\text{RVS}}<12$ &	>1	& $>30$ 			& 5\,600 &   & 6\,400 &  \\
%$G_{\text{RVS}}<12$ &	>2	& $>30$ 			& 4\,300 &   & 5\,000 &  \\
%$G_{\text{RVS}}<12$ &	>3	& $>30$ 			& 3\,200 &   & 3\,900 &  \\
%$G_{\text{RVS}}<12$ &	>6	& $>30$			& 1\,700 &   & 2\,100 &  \\
%\hline
%$G_{\text{RVS}}<12$ &	>0.5	& $>50$ 			& 4\,900 &   & 5\,600 &  \\
%$G_{\text{RVS}}<12$ &	>1	& $>50$ 			& 4\,900 &   & 5\,600 &  \\
%$G_{\text{RVS}}<12$ &	>2	& $>50$ 			& 4\,200 &   & 4\,900 &  \\
%$G_{\text{RVS}}<12$ &	>3	& $>50$ 			& 3\,200 &   & 3\,900 &  \\
%$G_{\text{RVS}}<12$ &	>6	& $>50$			& 1\,700 &   & 2\,100 &  \\
%\hline
%$G_{\text{RVS}}<12$ &	>0.5	&  \ \ $>100$ 		& 3\,900 &   & 4\,600 &  \\
%$G_{\text{RVS}}<12$ &	>1	&  \ \ $>100$ 		& 3\,900 &   & 4\,600 &  \\
%$G_{\text{RVS}}<12$ &	>2	&  \ \ $>100$ 		& 3\,800 &   & 4\,500 &  \\
%$G_{\text{RVS}}<12$ &	>3	&  \ \ $>100$ 		& 3\,200 &   & 3\,800 &  \\
%$G_{\text{RVS}}<12$ &	>6	&  \ \ $>100$		& 1\,700 &   & 2\,100 &  \\

%\hline                                             %inserts single line
%\end{tabular}
%\end{table*}







==> figures/Sec_BdDistribution.tex <==
%\subsection{Current models \label{sec:currentModel}}
%\subsection{Latest model \TODO{[set name]} \label{sec:latestModel}}
%As basis for our simulation we use the latest estimates from ....



==> figures/Sec_Conclusions.tex <==
%\EDIT{CAVEATS: we did not analyse false detection rates, i.e. contaminants.}

\EDIT{Based on detailed simulations, we find that \gaia is likely to detect tens of thousands of brown dwarfs from the astrometric data alone. From the \gaia radial velocity data alone there should be thousands of additional candidates, with a few hundred overlapping in the two domains. Photometric transits with S/N\,$>3$ are expected for perhaps a thousand systems, although with only tens or less overlapping with radial velocity or astrometric detections. Though the number of observations per source is typically only a few, they would be excellent targets for follow-up observations.

An extended mission of 10-years increases all of the detected numbers by 50--200\%, allowing the brown dwarf horizon to be extended even further. 
}

The numbers found in this study are ultimately limited in accuracy to about $\pm 50\%$ due to the presently uncertain occurrence rates and period distributions of brown dwarfs around FGK host stars.

The \gaia detections will enlarge the current brown dwarf sample by at least two orders of magnitude, and will allow for their characterisation in unprecedented detail, leading to a better understanding of the formation scenario of these FGK companions that populate the $10-80M_{\text{J}}$ mass range, and the exploration of the (perhaps not completely dry) desert within it.


==> figures/Sec_Discussion.tex <==
\subsection{Implications on understanding formation of massive planets and BDs \label{sec:implications}}
%\TODO{[TODO: Damien: add paragraph describing how GAIA will help constraining the formation scenario given the predictions of this paper.}

\gaia will detect several hundred of the most massive giant planets and brown dwarfs around solar type stars brighter than $G<10.2$. Combined with ground-based radial velocity follow-up observations, \gaia astrometry will allow the true mass of these companions to be derived, along with the corresponding orbital elements. These results will set the mass range at which the transition between the most massive planets and the least massive brown dwarfs occurs \citep{Sahlmann:2011yq}. In addition, the large sample size will provide detailed insight into the dependance of the occurrence of massive giant planets or BDs on the mass and or/the chemical composition of the host star. In turn, this will provide new constraints on both massive giant planets and BD formation theories.



%\subsection{Validation of expected number of BDs \label{sec:discussion:validation}}

%\subsubsection{Rough assumptions estimate}
%\TODO{[Useful?/Keep?]}
%Here we would like to make a rough validation of the expected number of BDs reported in Sect.~\ref{sec:results}. 
%Let's make the following assumptions:   
%\begin{itemize}
%\item the average FGK star has a mass of 1~$M_{\odot}$,
%\item the average FGK star has an eccentricity about 0.3 (50\% percentile of the pdf of Fig.~\ref{fig:eccDist}) for which the reduction in detection distance is around 4\% (Fig.~\ref{fig:gaiaDetecEcc}), resulting in a volume that is 0.88 ($0.96^3$) times that of a zero-eccentricity sample, 
%\item the average period of a BD is around 200--300~d ($\sim50\%$ percentile of Fig.~\ref{fig:cdfHistPeriodFit}, we will use here the 300~d from the Diaz distribution),
%\item $50\%$ has a mass of $15 M_{Jup}$ and 50\% a mass of $70 M_{Jup}$ (conform Fig.~\ref{fig:hollMassFunction}),
%having (zero-extinction, $\Delta \chi^2=100$) distance horizons of: 174~pc and 539~pc (conform Sect.~\ref{sec:gaiaResponseComp}),
%%\item From the \gaia sensitivity study of Sect.~\ref{sec:gaiaResponseComp} the corresponding zero-extinction $\Delta \chi^2=100$ distance horizons are: 174~pc and 539~pc (see also Fig.~\ref{fig:gaiaDetectability}),
%%quick and dirty estimate from http://www.pas.rochester.edu/~emamajek/memo_star_dens.html
%%F stars: 0.0025, G stars: 0.0048 , K dwarfs: 0.0135  per square parsec, sum = 0.0025+0.0048+0.0135 = 0.0208
%\item an average density of FGK stars in the solar neighbourhood to be 0.02 stars~pc$^{-3}$ (simply summing F: 0.0025, G: 0.0048 , K: 0.0135 stars~pc$^{-3}$) \TODO{[check number, add reference]},
%\item assuming this density for a uniform sphere for the $50\%$ of BDs of  $15 M_{Jup}$ up till 174~pc, and halving the count for a uniform sphere for the $50\%$ of BDs with $75 M_{Jup}$ that are detetable up till 539~pc (to compensate for the extend above and beyond the disk),
%\item  applying the adopted $0.6\%$ occurrence rate of BDs.
%\end{itemize}
%% take mean period of 300 d
%% hostmass=1, bd=15 mjup, ecc=0, period=300d, 174 pc (deltaChi2=100)
%% hostmass=1, bd=70 mjup, ecc=0, period=300d, 539 pc (deltaChi2=100)
%%0.02*0.006/2*4/3*pi*(174^3) = 1'323
%%0.02*0.006/2*4/3*pi*( 0.5*539^3) = 19'677
%%0.02*0.006/2*4/3*pi*(174^3 + 0.5*539^3) = 21'001
%% take mean period of 400 d
%% hostmass=1, bd=15 mjup, ecc=0, period=400d, 197 pc (deltaChi2=100)
%% hostmass=1, bd=70 mjup, ecc=0, period=400d, 571 pc (deltaChi2=100)
%%0.02*0.006/2*4/3*pi*(197^3 ) = 1'921
%%0.02*0.006/2*4/3*pi*(0.5*571^3) = 23'394
%%0.02*0.006/2*4/3*pi*(197^3 + 0.5*571^3) = 25'316
%% results times 0.88 due to the volume reduction of eccentricity 0.3:
%%0.96^3 * 0.02*0.006/2*4/3*pi*(174^3) = 1'171
%%0.96^3 *0.02*0.006/2*4/3*pi*( 0.5*539^3) = 17'409
%%0.96^3 *0.02*0.006/2*4/3*pi*(174^3 + 0.5*539^3) = 18'581
%
%This collection of assumptions for a 5-year mission and $\Delta \chi^2=100$ detection, leads to a number of 18.6~k expected BDs (1.2~k for the $50\%$ $15 M_{Jup}$ BDs, and 17.4~k for the $50\%$ $70 M_{Jup}$ BDs), consistent with the total number and mass-recovery reported in the results.


\subsection{Comparison with earlier work \label{sec:transit}}

\cite{Bouchy:2014aa} found that some 20\,000 BDs could be expected for bright $G_{\text{RVS}}<12$ host stars having radial velocity time series in \gaia, assuming they have:
\begin{itemize}
\item a $0.6\%$ BD occurrence rate (as assumed in this paper);
\item 3.4 million main sequence and sub-giants stars (total count from \cite{Robin:2012aa} for these luminosity classes);
\item a 100\% detection efficiency.
\end{itemize}


As described in Sect.~\ref{sect:resultsRv}, applying the limit of $G_{\text{RVS}}<12$ results in a sample of 1.8~million stars, which is only about half of those assumed in \cite{Bouchy:2014aa}. The difference is that in the latter, the selection is not constrained to be only FGK stars\footnote{We tried to extract the sample size of the FGK main sequence and subgiant with $G_{\text{RVS}}<12$ from the \cite{Robin:2012aa} catalog on Vizier, but unfortunately it does not contain the luminosity class.}. %\TODO{[I contacted Robin 2 weeks ago, but no answer..]}
% Robin 2012: G_RVS <12 type: F=13.83% G=15.46% K=41.75% = 71.04%
In \cite{Robin:2012aa} the fraction of FGK stars with $G_{\text{RVS}}<12$ is $71\%$ (20\% larger than expected from the discrepancy), though this is not limited to the aforementioned luminosity classes.

As mentioned in Sect.~\ref{sect:resultsRv} we find around 5000 BDs with a detection efficiency of about $30-50\%$ \EDIT{[Check and fix if needed]}.
Comparing this with the 100\% detection efficiency assumed in \cite{Bouchy:2014aa}, we can explain the discrepancy between their 20\,000 and our $\sim$5000~BDs: our sample is about half as large, and has a half as large detection fraction. Given that \cite{Bouchy:2014aa} did not constrain their estimate to FGK host stars, their BD number could be overestimated by a factor~2 when only considering the astrometric detection probability (which is closer to 50\% than 100\%). However, as it is expected there will be radial velocity time series available for $G_{\text{RVS}}<12$, the combined BD detection probability of these two methods could still turn out to be close to 100\%, and their estimate more realistic.

\cite{Bouchy:2014aa} also predicted a total of 60 transiting BDs for $G_{\text{RVS}}<12$. We predict \EDIT{about 35--120 BDs with transits when not accounting for any astrometric detection limit (see Table~\ref{tab:simResults}), which reduces to less than ten when we consider a minimum detectability limit of $\Delta \chi^2=30$. The numbers are therefore rather consistent.}

%Correcting for the factor of two in the number of sources, our prediction is either a factor 5 higher, or a factor of 2 lower than \cite{Bouchy:2014aa}, depending on whether we take into account the detectability or not. We ascribe these differences to the specific modelling applied, and conclude that generally we recover the same numbers within an order of magnitude.
%  to details of the modelling applied,We consider We   \TODO{for which we do not have an explanation, other than that the assumed transit probability per observation was probably chosen differently [I could go by, and ask Francois at the observatory about this]}.
%Note that when taking into account the detection thresholds, we predict the number of astrometric detected BDs around FGK hosts with $G_{\text{RVS}}<12$ having observable transits to be about 2.3, 1.7, and 1.2 for $\Delta \chi^2$ of 30, 50, and 100, respectively. This means that there might just be a few sources with both astrometric and radial velocity data.
% total sources up till G=12: 100*(619+1344+2230+3804) = 100*7'997 = 800'000 host stars.
%Bouchy : 0.2609*13 = 3.4 M (MS+SubGiant), difference of 4.25. 
%Figure~\ref{}

% Robin 2012: G_RVS <12  MS+subgiants: 3.4 M
% Robin 2012: G_RVS <12 type: F=13.83% G=15.46% K=41.75% = 71.04%
% so total around 3.4*0.71 = 2.414 M (though most are giants in distribution!)

% we find for Grvs<12 for FGK stars: 1,809,870 (~1%)


% MACP: can I suggest this section title
 \subsection{Estimates from a uniformly sample data set}
% \subsection{Bootstrapping with \cite{raimbault19} \label{sec:raimbaultBootstrap}}
In an attempt to estimate the number of expected BDs from a \textit{uniformly sampled dataset}, we used the Coralie survey dataset of \cite{raimbault19} in which about a hundred targets with companions having $2<M_{\text{J}} \sin i<433$ for a \textit{volume limited} sample are presented. Seventeen of these targets have $10<M_{\text{J}} \sin i<80$, of which two have $P\sim6$\,yr and one has $P\sim10$\,yr. As the latter will be hard to detect we remove it from the sample, but keep the two 6-year entries, i.e., a total sample of 16~BDs. We run additional simulation with this sample, but instead of sampling the companion mass, eccentricity, period, and period-eccentricity from our adopted CDF distributions, we bootstrap all our candidates from this sample (drawing samples with replacement). The comparison between the CDFs is illustrated in Figs.~\ref{fig:cdfHistPeriodFit}, \ref{fig:eccDist} and \ref{fig:pEcc}, showing that the \cite{raimbault19} distribution differs significantly from those derived from the \cite{2014MNRAS.439.2781M} and \cite{Diaz:2012aa} data. 

Note that we simply use $M_{\text{J}} \sin i$ as a proxy for $M_{\text{J}}$. The results are shown in Table~\ref{tab:RbsimResults}, indicating that the estimates would be 1.5--2 times higher than that using our adopted distributions (Table~\ref{tab:simResults}). Given that we adopted the \textit{minimum} mass estimate in our simulations, and the \gaia sensitivity is higher for more massive companions, this might suggest that if the Raimbault sample is representative for the real BD distribution, we could expect up to twice as many BDs as suggested in Table~\ref{tab:simResults}. 
%\TODO{[Looking at the Fig.~\ref{fig:perDistRb} shows that the period cdf is not very nice and could probably easily cause the large excursion from the rest of our results. Given that rather small sample size I suggest NOT to include this section in the paper, as it is not very consistent with the previous results and unclear if it is more significant than what we alraedy presented. ]}
%(sep<5 AU, SN50>50, contrast CCF>30, svrad>0.01, fwhm<14km/s, LogR'HK<-4.75, Msini>1 MJup).

\begin{table}[t]
\tiny
\caption{Simulation results from bootstrapping with a BD sample from \cite{raimbault19}. The number of detected BDs is tabulated, with in parentheses the number of host stars having \EDIT{individually detectable photometric transits in \gaia data (S/N>3)} together with their mean number of transits. \EDIT{The period distributions `Raimbault' is shown in Fig.~\ref{fig:cdfHistPeriodFit}. All counts could be up to $50\%$ higher or lower due to the uncertainty on the assumed $0.6\%$ BD occurrence rate (see Sect.~\ref{sec:bdFractHostStars}).}} 
\label{tab:RbsimResults}  
\centering    
%\renewcommand{\arraystretch}{1.0}                    
\begin{tabular}{c@{\kern0.7em}  c@{\kern0.7em}  c | r @{\ }l | r@{\ } l  }          % 
\hline\hline      
Magnitude & Astro & RV & \multicolumn{2}{c|}{5-yr nominal} & \multicolumn{2}{c}{10-yr extended} \\
%\cline{2-5}    
selection & $\Delta \chi^2$ & $\Delta \chi^2$ & \multicolumn{2}{c|}{$\text{P}_\text{distr}$ = Raimbault} & \multicolumn{2}{c}{$\text{P}_\text{distr}$ = Raimbault} \\    % table heading
\hline                                 
--                 & -- 	        & --	& 780\,000 	&(810: 1.6)    & 780\,000 &(1300: 1.8) \\
\hline
--                 & $>30$         & --	    & 60\,000 & ( \   21: 1.5)   & 100\,000 & ( \ \ \  77: 1.8)  \\
--                 & $>50$         & --	    & 42\,000 & ( \   13: 1.4)  & 74\,000 & ( \ \ \  46: 1.6)  \\
--                 & \ \ $>100$    & --	    & 26\,000 & ( \ \ \   7: 1.4)  & 48\,000 & ( \ \ \  23: 1.4)  \\
\hline
\hline
$G_{\text{RVS}}<12$ & -- 		    & --	& 12\,000 & ( \     35: 1.7)  & 12\,000 & ( \ \ \ 58: 2.0)	 \\ 
\hline
$G_{\text{RVS}}<12$ & $>30$ 		& --	& 8200 & ( \  12: 1.6)  & 9700 & ( \ \ \ 33: 2.0)	 \\ 
$G_{\text{RVS}}<12$ & $>50$ 		& --	& 7200 & ( \ \ \   7: 1.6)  & 8700 & ( \ \ \ 23: 1.9)	 \\ 
$G_{\text{RVS}}<12$ & \ \  $>100$ 	& --	& 6000 & ( \ \  \ 4: 1.5)  & 7500 & ( \ \ \ 13: 1.8)	 \\ 
\hline
$G_{\text{RVS}}<12$ & --	        & $>30$     & 1800 & ( \  22: 1.7)  & 3100 & ( \ \ \   47: 2.1) \\
$G_{\text{RVS}}<12$ & --	        & $>50$     & 1000 & ( \  15: 1.7)  & 2000 & ( \ \ \   38: 2.1)  \\
$G_{\text{RVS}}<12$ & --	        & \ \ $>100$& 450 & ( \ \ \  8: 1.8)  & 1000 & ( \ \ \   24: 2.2) \\
\hline
$G_{\text{RVS}}<12$ & $>30$	        & $>30$     & 1100 & ( \ \ \  9: 1.6)  & 2400 & ( \ \ \   29: 2.0)  \\
$G_{\text{RVS}}<12$ & $>50$	        & $>50$     & 550 & ( \ \ \  4: 1.6)  & 1300 & ( \ \ \  17: 2.0)  \\
$G_{\text{RVS}}<12$ & \ \ $>100$	& \ \ $>100$& 190 & ( \ \ \  2: 1.6)  & 560 & ( \quad \  7: 1.9)   \\

\hline                                             %inserts single line
\end{tabular}
\end{table}



% Suggested to not include
%
%\subsection{Validating the magnitude host star distribution as function of magnitude\label{sec:hostAssesment}}
%\TODO{[This section is meant to asses the precision of teh Besan\c con model counts as function of magnitude.  We can use \gaia DR2 data where we can get good estimates of the numbers, if the BSC model numbers line up with the \gaia number of host stars per magnitude bin. The main problem is to be able to select only the main sequence and sub-giants, for which we could use an absolute magnitude cut as function of $T_{\text{efff}}$ (or BP-RP), for which we need accurate parallaxes.
%Some \gaia extraction was started initially, added to Appendix~\ref{sec:gaiaDR2}.] Perhaps this idea is too detailed to include but I was thinking of the following validation:
%\begin{itemize}
%\item we try to select parts of the data in magnitude bins that we can compare between \gaia DR2 and the used BSC model. E.g. we can easily select in \gaia DR2 magnitude bins.
%\item we can assume that on average the effective temperatures in \gaia DR2 are sort of ok and extract the count within a certain range for FGK-stars, though we would not account for any extinction.. 
%\item we can use Fig.~\ref{fig:accParError} to select a certain magnitude error, to cut (for a certain magnitude bin) a sample of \gaia data with very precise parallaxes, which is a representative sample of all sources (and distances) in that magnitude bin. This only works if the parallax error is independent from the parallax, which we can easily check by plotting one against the other (TODO). 
%\item If this is the case we can use the parallax to compute the absolute magnitude and apply a cut that would keep only the main sequence and sub-giants, and then count the \gaia sources per magnitude bin of this subsample, and scale it back to the full size by using the fraction of the sample wrt to the total in the magnitude bin. 
%\item We can compare this against the counts for the same magnitude cut in the BSC model, and plot the ratio per magnitude bin. This should be around 1, though it would be good how large, and in which directions there are deviations, which we can use then in our conclusions to say something more about the uncertainty on our estimate.
%\item probably we can use this trick up to magnitude 17 (which probably is sufficient to validate the bulk of our data given the histogram of Fig.~\ref{fig:magHist}) where $T_{eff}$ is no longer available in \gaia data. Alternatively we can some BP-RP colour (I computed it for the BSC model data already), though again, taking into account extinction would make the \gaia query non-trivial, so we should probably neglect that. 
%\end{itemize}
%}
%
%\begin{figure}[h]
%%  \vspace{0cm}\\
%  \includegraphics[width=0.49\textwidth]{figures/DR2astrometricPrecision_v3.pdf} 
%\caption{Distribution of DR2 \gaia astrometric errors. Assuming they are independent of parallax (we can easily check by plotting one vs the other), we can use this to select a sub-sample of source with very precise parallax so that we can apply a distance cut in \gaia data and BSC data for a certain magnitude, and compare the counts. }
%\label{fig:accParError}
%\end{figure} 





%\subsection{Missing BDs around bright stars with G<10.2\label{sec:missingBrightHost}}
%In Sect.~\ref{sec:besancon} we identified that the Besan\c con model does not produce any output below G-band magnitude 10.2, while the detection should be rather complete as seen from the increasing recovery fraction of Fig.~\ref{fig:magHist}, which is 50\% and higher for G<12. To identify if this omission is significant for our estimation we will make a rough calculation of how many we might be missing. First of all we simply query the approximate amount of FGK stars in \gaia DR2 with mean G<12.2, by using the rough limits: of $4000 < T_{\text{eff}} <7200$, not accounting for any (local) extinction or quality flags that might indicate errors in the effective temperature \TODO{[TODO: this did NOT yet filter only the main sequence and sub-giants!! Should we assume a certain fraction? Or make an absolute magnitude cut, which then only works properly for the most significant parallaxes (in DR2 around G=12 90\% of sources has \texttt{parallax\_over\_error} > 10, 95\% has \texttt{parallax\_over\_error} > 5]}:
%\begin{verbatim}
%select count(*) from gaiadr2.gaia_source 
%where phot_g_mean_mag<=10.2  
%and teff_percentile_lower>4000  
%and teff_percentile_upper<7200 \end{verbatim} 
%resulting in 388\,636 sources (527\,293 when using $G<10.5$). Assuming the same 0.6\% BD fraction as in the rest of this study we have around 2300 BDs, the majority being towards the G=12 faint end. Assuming an average detection fraction of 0.6  for the most solid detection (having $\Delta \chi^2>100$), we might have missed around 1400 BDs on a number of 16\,000, meaning an underestimation of about 10\%. For the marginal detections (having $\Delta \chi^2>30$) we could assume an average detection fraction of 80\%, which would mean an underestimation of about 1900 BDs on the estimated 38\,000, which would be around 5\%.  From this we conclude that although these bright targets are obviously the most interesting for follow-up studies, they do not bias our total number estimate significantly. \TODO{[is obviously less when we filter on MS and subgiants! Should we run a quick simulation e.g. on Hipparcos sources??? or the above selected \gaia sources, as they will mostly have good distance estimates, and else we could use the CBJ bayesian distance prior?.]}




%\subsection{Transiting brown dwarfs from \gaia astrometry \label{sec:transit}}


%\TODO{[COMPARE ALSO TO Perryman (2014) paper! (any suggestions exactly what to compare?)]}

==> figures/Sec_GaiaDetectionLimits.tex <==
% MACP: I suggest that the introduction should be re-written to stress the applicability of the method to NS and WD.

\label{sec:gaiaResponseComp}
%\subsection{\EDIT{astrometric} detection limits}
\EDIT{This Section is intended to provide insight in the astrometric detection limit by means of simulating a large-grid of models. Note that this data was not used in any of the computations of this paper, and just serves as illustration for the reader.}
%\EDIT{mention this data was only generated for the illustration of the sensitivity of the method.}



\EDIT{[NEEDED, ANYWHERE?] For completeness we wish to convey that the astrometric sensitivity of \gaia to detect unseen companions has been assessed in literature in various publications for the per-transit `S/N statistic' (as well as for non-\gaia radial velocity data) \cite[see e.g.][]{Casertano:2008aa,2010EAS....45..273S, 2010EAS....42...55S,2014EAS....67...93S, 2014MmSAI..85..643S}. This statistic compares the astrometric signature  $\alpha_*$ of the host star\footnote{Astrometric signature in arcsec: $\alpha=(M_\text{BD}/M_{*})(\overline{a}_{\text{BD}}/d)$ where $M_{\text{BD}}$ is the (unseen) BD companion mass, $\overline{a}_{\text{BD}}$ its semi-major axis in au, and $d$ the distance in pc to the system.}, against the (typical) accuracy of an individual epoch, $\sigma_{\text{fov}}$.}


 








The \gaia  astrometric detection limits of a specific binary companion depend on the time sampling and astrometric error model, detailed in Appendices~\ref{sec:gaiaTs} and ~\ref{sec:gaiaError}, respectively. Provided with these, we can construct the detection limits as a function of the companion orbital parameters. Below we detail the resulting behaviour.
%, of which the numbers are tabulated in Appendix~\ref{sec:responseFunctionResults}.


For a given host mass ($M_{\text{*}}$ in $M_{\odot}$) and absolute magnitude ($G^{\text{abs}}_\text{*}$), and companion mass ($M_{\text{BD}}$), eccentricity ($e$), period ($P$ in days), and distance ($d$ in pc) we make $2\times 784$ simulations: for 784 HEALPix sky-uniform distributed time series (see Appendix~\ref{sec:gaiaTs}) we sample the time series for both a 5-yr and 10-yr mission, with each observation being subject to a random rejection probability of $\sim$10\% to simulate dead time. 

The reference time for the astrometric model, $t_{\textrm{ref}}$, is set to the middle of the selected time series. From the parallax ($\varpi$ in arcsec = 1/distance in pc) and $G^{\text{abs}}_\text{*}$ we compute the apparent G-band magnitude of the host star assuming zero extinction: $m_\text{*}= G^{\text{abs}}_\text{*} - 5 (\log10(\varpi) + 1)$, 
%\footnote{To be precise, the calculations for this response function are based on the parallax, which is represented for the users convenience as distance (pc) and apparent G-band magnitude assuming zero extinction.}),
 which is used to extract the astrometric error on the observations using Eq.~\ref{eq:fovPrecision}. 
 
The companion-to-host semi-major axis ($\overline{a}$ in au) is computed from the period and sum of the masses using Kepler's third law: $\overline{a} = P^2 (M_\text{*} + M_{\text{BD}} )^{1/3}$ \EDIT{[TODO: FIX formula]}. The sky-projected semi-major axis ($a_\text{*}$~in~arcsec) of the host star with respect to the system barycentre is computed from $\overline{a}$, the parallax,  and mass ratio ($q=M_{\text{BD}}/M_{\text{*}}$) as:
 %\footnote{\TODO{[Footnote for co-authors: I think I got it right but good to verify above equations. Note that when we would have used the baricentric planet semi-major axis $\overline{a_{bd}}$ the latter formula would have been as Eq. 6 of Perryman (2014):  $a_\text{*}=\varpi \overline{a_{bd}} q $, because $\overline{a}_\text{*}/\overline{a}_{\text{BD}}=M_{bd}/M_\text{*}$ . By the way, do you think it is more useful to tabulate $\overline{a}_{\text{BD}}$ (i.e. the semi-major axis wrt to barycentre, named $a_\text{p}$ in Perryman (2014)), instead of $\overline{a}$?]}}: 
 $a_\text{*}=\varpi \overline{a} q / (q+1)$. The orientation of the companion is randomly drawn in 3d space, i.e., inclination, argument of periapsis, position angle of the receding node, and mean anomaly at $t_{\textrm{ref}}$. For each simulation the centrality parameter $\lambda$ (Sect.~\ref{sec:gaiaDetectMethod}) is computed. 
%mass ratio ($q=M_{\text{BD}}/M_{\text{*}}$)

In a next step, for the 5- and 10-yr simulations separately, we compute the fraction of the 768 simulations for which $\lambda>23, 43, 93$, i.e.\ the fraction of simulations corresponding to $\Delta \chi^2>30,50,100$. The 768 simulations uniformly cover the whole sky and each have a random orbit orientation, hence this fraction can be considered a `sky average' value. 

\begin{figure}[b!]
 \includegraphics[width=0.49\textwidth]{figures/sensitivity/G2V_10Mj_4y_GaiaResponseEcc.pdf}  
\caption{Eccentricity dependence of distance and magnitude detection limits for $\Delta \chi^2=100$ for a G2V star and a $10M_{\text{J}}$ BD with $P=4$\,yr. The black point at $e=0$ corresponds to the black point in the middle panel of Fig.~\ref{fig:gaiaDetectability}. Sky-detection fractions of 50 percentile (thick line) and 10--90 percentile (shaded region) illustrate that the detection threshold for such a (randomly oriented) system varies by $\pm25\%$, depending on sky position. %the zero-eccentricity value dot corresponds to the dot in the middle panel of Fig.~\ref{fig:gaiaDetectability}. \TODO{[update figure with latest, has 20\% variance]}
}
\label{fig:gaiaDetecEcc}
\end{figure} 


To tabulate and plot the response as function of period (or semi-major axis) as shown in Figs.~\ref{fig:gaiaDetecEcc} and \ref{fig:gaiaDetectability}, we compute these statistics for a range of logarithmically increasing distances and identify (interpolate) the distance of the 10\%, 50\%, and 90\% sky-detection fraction of the various $\lambda$ thresholds. 
%To get the response we interpolate for a set of period steps the location where $\lambda=23, 43, 93$, i.e., corresponding to $\Delta \chi^2=30,50,100$.
% 4yr (=1461d) actual data: 1468 d,  
% deltaChi2=100: 10%=356.34 (22%) 50%=292.97 90%=224.31 pc (-23%)
% deltaChi2=50: 10%=459.04 (21%) 50%=379.71 90%=304.83 (-20%) pc
% deltaChi2=30: 10%=558.91 (19%) 50%=469.18 90%=387.89 (-17%) pc
%From sim9 ecc file:
% deltaChi2=30: 10%=352.02 (15%) 50%=305.54 90%=260.47 (-14%) pc

The results of the 50\% sky recovery fraction is shown by the lines in Figs.~\ref{fig:gaiaDetecEcc} and \ref{fig:gaiaDetectability} , while the 10\% and 90\% fractions are used to draw the shaded range in Fig.~\ref{fig:gaiaDetecEcc}. For example: the black dot in both figures is a BD companion around a G2V star (1~$M_{\odot}$) with a zero eccentricity BD of mass $10M_\text{J}$, having $P=4$~yr, observed during a 5-yr nominal mission. It will have a good orbit recovery ($\Delta \chi^2=100$) for 50\% of the sky at 311\,pc. The distance range corresponding to the $10\%$ and $90\%$ sky coverage for this recovery is 381--234~pc, i.e.\ $\pm \sim 25\%$ visualised by the shaded range at eccentricity zero of Fig.~\ref{fig:gaiaDetecEcc}. 
As eccentricity increases, the detection efficiency slowly decreases, resulting in a distance limit about 10\% lower around $e=0.5$, and reaching more than 20\% lower for $e>0.7$. Given the significant eccentric distribution of BDs (see Sect.~\ref{sec:eccVsPeriod}) the overall effect is non-negligible. The solid line is similar for other periods of this system, though the  $10\%$--$90\%$ sky coverage range increases for shorter periods: e.g., to $\pm$45\% for $P=1$~yr. Comparing this to a 100~$M_\text{J}$ companion, the 50\% sky fraction solid line drops below 20\% for $e>0.8$, while the $10\%$--$90\%$ sky coverage range expands from $\pm 15\%$ to some $\pm25\%$ for $P=4$ to $P=1$\,yr.

Fig.~\ref{fig:gaiaDetectability} demonstrates that detectability increases for increasing period, which can be understood through Kepler's third law: the (projected) semi-major axis increases as a function of period, hence boosting detectability. The peak occurs around the mission length, and as discussed in Sect.~\ref{sec:gaiaDetectMethod}, periods (much) beyond the mission length are increasingly difficult to recover, and good parameter recovery is no longer connected to the adopted $\Delta \chi^2>100$. To make this clear, this region is shaded in the plots.

The adopted accuracy floor for $G<12$ (see Fig.~\ref{fig:FovAccLaw} of Appendix~\ref{sec:gaiaError}) leads to a different slope of the detectability curves of Fig.~\ref{fig:gaiaDetectability} for distance $<800$, $<300$, and $<85$~pc, for the shown F0V, G2V, and K6V host star, respectively. Thus, for the $G<12$ regime %all measurements have basically the same astrometric precision, independent of the host apparent brightness, and hence 
the difference in detectability between host stars is only dependent on $q$, which for a given $M_{\text{BD}}$ is higher for late-type stars. 
As the detectability of a 1~$M_{\textrm{J}}$ companion lies within the $G<12$ regime, this translates into the further distance limit for the 1~$M_{\textrm{J}}$ companions for a K6V host compared to a F0V host, as seen in Fig.~\ref{fig:gaiaDetectability}.

For parts of the curves that are in the  $G$>$(\gg)12$ regime, the astrometric error is strongly dependent on apparent magnitude (Fig.~\ref{fig:FovAccLaw}), which effectively `outweighs' the smaller mass ratio for heavier stellar host mass, and hence produces a larger astrometric signal for earlier type stars, e.g.\ as seen in the further distance limit of the peak of a $100M_{\textrm{J}}$ companion for a F0V star compared to a K6V.


%Comparing the different host masses (and their corresponding absolute magnitude) we see that for decreasing host mass the distance limit for a $100M_{\textrm{J}}$ companions  goes down, while for the very light $1M_{\textrm{J}}$ companions it goes up. The reason is a combination of astrometric error model (which is flat below G<12, see Sect.~\ref{sec:gaiaError}), and the apparent magnitude (determined by their distance and absolute magnitude). Specifically, one can see that in all three examples the $1M_{\textrm{J}}$ companion is below G=12 and hence the astrometric signal is only dependent on the mass ratio  $q=M_{\textrm{bd}}/M_{\textrm{*}}$, which increases for lighter stellar host mass, and hence boosts detectability. For the $100M_{\textrm{J}}$ companion most of the curve has G>12 and hence the astrometric error is heavily dependent on apparent magnitude, which effectively `outweights' the smaller mass ratio for heavier stellar host mass and hence produces a larger astrometric signal for heavier hosts. The peak of $10M_{\textrm{J}}$ lies somewhere in the transition zone and hence does not change too much for different host masses.


In summary: 
(1)~for a given host and BD mass the detectability increases with period and reaches maximum sensitivity for periods close to the mission length;
(2)~orbital parameters of systems with periods (well) beyond the mission length are not recovered;
(3)~increased eccentricity reduces detectability;% with distance limits reduced to $-20\%$ ($\sim$ -0.5--0.7~mag) or less beyond 0.7--0.8). 
(4)~for a given companion mass, companions around earlier type stars are detectable at larger distances when $G>12$ 
%beyond a distance of $\sim200$~pc 
due to the higher intrinsic brightness of the host star and the specific \gaia magnitude dependent accuracy, despite the smaller mass ratio.
% OLD UNCLEAR \item for a given companion mass, the detectability of companions around earlier type stars is higher beyond a distance of $\sim200$~pc due to the higher intrinsic brightness of the host star and the specific \gaia magnitude dependent accuracy, despite the smaller mass ratio.

 \EDIT{[include or not? or perhaps for relevant WD, NS and BH mass] Apart from simulating detection limits for the BD mass range, it was a small effort to simulate these limits for a  larger range of (unseen) companion masses are presented in Fig.~\ref{fig:gaiaDetectabilityMassive}.}
 
 


%This behaviour in eccentricity and sky-fraction range as shown in Fig.~\ref{fig:gaiaDetecEcc} is typical for all points along the curves of Fig.~\ref{fig:gaiaDetectability} when the period is shorter than the mission duration. 
%\TODO{[Check if this is indeed correct.]}

%Typical relative change in detection distance and observed magnitude with respect to the zero-eccentricity data of Fig.~\ref{fig:gaiaDetectability}, illustrating that more the sensitivity drops for increasing eccentricity.
%Besides the 50 percentile (thick line), the shaded region illustrates the 10-90 percentile sky-detection fraction, illustrating that the detection threshold for a system can vary by $\pm20\%$ depending on its position on the sky. This is a typical curve for periods shorter than the mission length. The actual data shown is for a BD with 10 M$_{J}$, a 4 year period, around a solar-type host star, for a 5-year nominal mission; the zero-eccentricity value dot corresponds to the dot in the middle panel of Fig.~\ref{fig:gaiaDetectability}.

%Tables with these simulated detection limits are part of the electronic material of this paper (Appendix~\ref{sec:responseFunctionResults}). Note that in all further results presented in this paper the $\lambda$-values are computed directly for the relevant systems and not interpolated from these tables.

\begin{figure*}[ht!]
%\begin{tabular}{@{}lll@{}}
%\setlength{\tabcolsep}{0pt} % General space between cols (6pt standard)
%\renewcommand{\arraystretch}{0} % Ge\vspace{-0.08cm} \\neral space between rows (1 standard)
%%  \vspace{0cm}\\
% \includegraphics[width=\textwidth]{figures/sensitivity/3axis_ecc0_hostF0.pdf}  \\[6pt]
% \includegraphics[width=\textwidth]{figures/sensitivity/3axis_ecc0_hostG2V.pdf}  \\[6pt]
% \includegraphics[width=\textwidth]{figures/sensitivity/3axis_ecc0_hostK5.pdf}  \\[6pt]
%\end{tabular}
%  \vspace{0cm}\\
 \includegraphics[width=\textwidth]{figures/sensitivity/F0V_3axis_ecc0_host.pdf}  
% \hspace{0.9cm}\\
 \includegraphics[width=\textwidth]{figures/sensitivity/G2V_3axis_ecc0_host.pdf} 
%  \hspace{0.9cm}\\
 \includegraphics[width=\textwidth]{figures/sensitivity/K6V_3axis_ecc0_host.pdf} 
\caption{\gaia detection limits for a $100M_{\textrm{J}}$, $10M_{\textrm{J}}$, and $1M_{\textrm{J}}$ unseen companion around a F0V/G2V/K6V main sequence star (top/middle/bottom respectively) for  different $\Delta \chi^2$ detectability thresholds (see Sect.~\ref{sec:gaiaDetectMethod}) resulting from a simulated 5-year nominal mission (left) and 10-year extended mission (right). The lines shows the zero-extinction limits in distance (left axis) and apparent G-band magnitude (right-axis) for which 50\% of the simulated sky positions stops to be detectable at the given $\Delta \chi^2$. Note that the furthest distance limits occur at the simulated mission length of five and ten years. The eccentricity dependence and sky-position variation for the dot in the middle panel is expanded in Fig.~\ref{fig:gaiaDetecEcc}, see Sect.~\ref{sec:gaiaResponseComp} for more details. In the shaded regions the orbital parameters are no longer correctly recovered, see Sect.~\ref{sec:gaiaDetectMethod}. The semi-major axis $\overline{a}$ between the host and unseen companion, corresponding to a given period, is shown above the graph. For the shown low mass ratios this scale is practically the same (in contrast to that of massive unseen companions shown in Fig.~\ref{fig:gaiaDetectabilityMassive}). \EDIT{[TODO: trim x-axis to 5 and 10 year!]}
}
\label{fig:gaiaDetectability}
\end{figure*} 


%\TODO{[PERHAPS CHANGE FIGURES AND ABOVE EXAMPLE FOR 80 $M_{J}$ upper limit?]}.

%\TODO{[I suggest we append an electronic table to this paper with the sensitivity numbers (I spent quite some time on it anyway), for a whole range of unseen companion masses, up to q=10 for example, so that people who do studies of neutron-star/black-hole binaries can directly use these sensitivity curves. Current literature assumptions about Gaia sensitivity for these objects as function of period are very poor, as mentioned in the introduction of Sect.~\ref{sec:gaiaSensitivity}.]}.




 %\TODO{[Perhaps move this discussion with table preview to Appendix?] 

 
%These data are thus applicable beyond the BD scope of this paper, for example in the study of \gaia detection of faint (dormant/non-active) but heavy companions, such as white dwarfs, neutron stars, or black holes. Existing studies by \cite{Mashian:2017aa, Breivik:2017aa, Yamaguchi:2018aa}  (necessarily) had to make various assumptions about the \gaia sensitivity function, but could possible profit from these estimates in future work. When using these data, one should take into account that it is based on the assumptions that: 1) the host star light has undergone no extinction, 2) the system follows a strictly Keplerian orbit, 3) the companion is completely dark, i.e., it is sufficiently fainter than its host star that its light does not influence the astrometric (centroiding) measurement, and 4) there are no additional effects simulated that could perturb the photocentre motion of the specific host star types (e.g. spots). Additionally, when used to assume orbital parameter recovery for $\Delta \chi^2>100$ one should not use these data for periods (much) beyond the simulated mission lengths, as explained in Sect.~\ref{sec:gaiaDetectMethod}.

\begin{figure*}[ht!]
 \includegraphics[width=\textwidth]{figures/sensitivity/F0V_massive3axis_ecc0_host.pdf} 
 %\vspace{0.01cm}
 %\\
 \includegraphics[width=\textwidth]{figures/sensitivity/G2V_massive3axis_ecc0_host.pdf} 
  %\vspace{0.01cm}
  %\\
 \includegraphics[width=\textwidth]{figures/sensitivity/K6V_massive3axis_ecc0_host.pdf} 
\caption{
\gaia detection limits for a \textbf{massive} $100M_{\odot}$, $10M_{\odot}$, and $1M_{\odot}$ unseen companion around a F0V/G2V/K6V main sequence star (top/middle/bottom respectively) for  different $\Delta \chi^2$ detectability thresholds (see Sect.~\ref{sec:gaiaDetectMethod}) resulting from a simulated 5-year nominal mission (left) and 10-year extended mission (right). The lines shows the zero-extinction limits in distance (left axis) and apparent G-band magnitude (right-axis) for which 50\% of the simulated sky positions stops to be detectable at the given $\Delta \chi^2$. Note that the furthest distance limits occur at the simulated mission length of five and ten years and beyond them the orbital parameters are no longer correctly recovered (shaded), see Sect.~\ref{sec:gaiaDetectMethod}. Also, magnitudes fainter than the \gaia limiting magnitude of $G=20.7$ are shaded.   The semi-major axis $\overline{a}$ between the host and unseen companion, corresponding to a given period, is shown below the graph for each companion mass. ( For the detectability curves of low mass unseen companions see Fig.~\ref{fig:gaiaDetectability}.).}
\label{fig:gaiaDetectabilityMassive}
\end{figure*} 

==> figures/Sec_GaiaSensitive.tex <==

\EDIT{The most fundamental factor in estimating the expected number of brown dwarfs by \gaia is to quantify what we call a `detection'.} We define this for astrometry in Sect.~\ref{sec:gaiaDetectMethod}, for radial velocity in Sect.~\ref{sec:gaiaDetectMethodRv}, and for photometric transits in Sect.~\ref{sec:gaiaDetectMethodTransit}.
\EDIT{We do not attempt to quantify false-detection rates for the various thresholds, as this will be strongly dependent on the noise properties and remaining `features' in the final data.}
 
%, and (2)  the resulting  \gaia  detection limits as function of companion orbital parameters, described in Sect.~\ref{sec:gaiaResponseComp}. 
 
 
\subsection{\EDIT{Astrometric} detection criteria \label{sec:gaiaDetectMethod}} 
% MACP: this para moved from Section1
The high accuracy astrometric measurements of \gaia \citep{2001A&A...369..339P,Lindegren:2012aa, Lindegren:2016qy, Lindegren:2018aa, 2020arXiv201203380L} are key to the astrometric detection of brown dwarf companions, and indeed unseen companions in general. 
\EDIT{ For a circular orbit and small mass ratio \cite[][Eq.~3.2]{2018exha.book.....P}}
\begin{equation}
\alpha =
\left( \frac{M_p}{M_{*}} \right)
\left( \frac{a}{1~\text{AU}} \right)
\left( \frac{1~\text{pc}}{d} \right) 
\text{arcsec} \ .
\end{equation}
This astrometric signal increases linearly with semi-major axis $a$ of the companion, such that wider orbits, and longer periods, yield a larger signal. \EDIT{However, the signal decreases linearly with increasing distance, so that detections will be dominated by relatively nearby stars.}

\EDIT{The astrometric detection method used here is adopted from \cite{2014ApJ...797...14P}, where it was used to assess the number of planets detectable with \gaia. It is based on the  astrometric $\Delta \chi^2 = \chi^2_{\mathrm{min}}\hbox{(5 parameter)} - \chi^2_{\mathrm{min}}\hbox{(12 parameter)}$, i.e., the difference in $\chi^2$ between a single-star astrometric model fit to the observations (having 5 parameters) and a Keplerian orbital fit to the observations (having 12 parameters). As $\Delta \chi^2$ is sensitive to the number and distribution of observations, the eccentricity and inclination of the system, and orbital period in relation to the total length of the observations, it can serve as a precise estimate of detectability once the relevant thresholds have been calibrated.

Following the findings resulting from the simulations in \cite{2014ApJ...797...14P}, we adopt their three thresholds for $\Delta \chi^2$:
\begin{enumerate}
\item $\Delta \chi^2 \simeq 30$ is considered a marginal detection, % (theoretically false detection $\sim 10^{-4}$),	% MACP suppressed
\item $\Delta \chi^2 > 50$ is generally a reliable detection,
\item $\Delta \chi^2 > 100$ generally results in orbital parameters determined to 10\% or better. 
\end{enumerate}
This procedure can be applied to both real and simulated data. 
However, the drawback of this $\Delta \chi^2$ detection metric is that it is computationally expensive to find the best 12-parameter Keplerian solution for millions of astrometric time series. For simulation work, Sect.~5 of \cite{2014ApJ...797...14P} provides however an elegant shortcut through the introduction of the \textit{noncentrality} parameter $\lambda$, which is simply the 5-parameter $\chi^2_{\mathrm{min}}\hbox{(5 parameter)}$ fit to the \textit{noiseless} data, and thus is applicable to simulations only. 

For the astrometric $\Delta \chi^2$ the difference in number of parameters between the 5- and 12-parameter model is~7;  therefore $\lambda+7$ approximates the expectation value of $\Delta \chi^2$ \citep[][Appendix~B]{2014ApJ...797...14P}. Note that this estimate does not include any statistical variance that would be induced by observation noise. This can easily be re-introduced by randomly drawing from the expected variance distribution around the predicted $\Delta \chi^2$. 

For the adopted thresholds in this paper these distributions are largely symmetric, and thus any biases when omitting this `noisification' of our large number of (and randomly initialised) samples is expected to be negligible. In this paper, as in \cite{2014ApJ...797...14P}, this noisification step was omitted, and for each star in our simulation we therefore only need to generate a noiseless astrometric signal representing the true orbit, compute the $\chi^2$ of a 5-parameter fit, and add~7 to determine the (noiseless) $\Delta \chi^2$ astrometric detection statistic\footnote{\EDIT{Though some computational cost is involved in simulating the orbital signal of a Keplerian system and making a 5-parameter solution to it, it is \textit{much cheaper} than taking the average of a large number of Keplerian 12-parameter solutions to Monte Carlo noise realisations of the same signal, while providing basically the same information.}}.

}

\subsubsection*{\EDIT{Validity of the $\Delta \chi^2$ thresholds}}
The quality indicators associated with $\Delta \chi^2 \simeq30$, 50, and 100 are only valid when the period $P\lesssim$ simulated mission length $T$, i.e., for (somewhat) longer periods the orbital parameters will no longer be recovered, even when $\Delta \chi^2 > 100$. This is because for $P<T$ the orbital signal has typically a low correlation with any of the 5~astrometric parameters because of its oscillating (periodic) nature. Consequently, it does not get absorbed in (and biasses) any of the positions, parallax\footnote{An exception to this are systems with an orbital period very close to the 1 year parallactic motion, see \cite{2000fepc.conf..479L,Butkevich:2018aa,   2010IAUS..265..416S} for more detailed discussions.}, or proper motions efficiently.  Instead, the orbital signal remains largely unmodelled, and ends up as an increased variance in the residuals. It increases the $\chi^2$, allowing us to use it as a measure of the difference (and hence detectability) between the 5-parameter single star solution, and the 12-parameter orbital solution. 

In the regime $P>T$, the longer the period, the smaller the section of the orbit that is probed. For longer periods, this curved orbital segment more closely resembles a contribution to the proper motion, resulting in biassed estimates of the proper motion. This then reduces the residual of the 5-parameter solution, and hence the $\chi^2$. Orbital fitting tests show that the period recovery starts to drop significantly beyond $P\sim T$, hence the $\Delta \chi^2$ thresholds no longer correspond to a well-defined quality of the parameter fits. Results from planetary mass companion fitting for a 5-year mission shows that periods are not properly recovered beyond 6--6.5~years \citep[][Fig.~6]{Casertano:2008aa}, though for BDs or heavier unseen companions  this may be extended to some 10~years or more. \EDIT{In this paper we will generally not consider periods beyond the simulated mission lengths of 5 and 10~years, as this would require actual orbital fitting. As will be discussed in Sect.~\ref{sec:bdPriors}, the BD period distributions used in this study are limited to $P<5$~yr (due to poor literature constraints for longer periods), which justifies the use of our detection method to give meaningful statistics for the whole simulated sample.}
%
For the recovery of an acceleration model instead of an orbital model, the  $\Delta \chi^2 > 100$ might still be considered a good criterion for $P>T$.

In summary, for $P\lesssim T$, higher values of $\Delta \chi^2$ give both more reliable detections and higher precision of the estimated orbit. 
In this paper all \EDIT{noiseless} $\Delta \chi^2$ values are approximated by the use of the non-centrality parameter $\lambda$  via the relation $\Delta \chi^2=\lambda+7$. 
%All of the results in this paper are expressed with respect to these limits and are derived from the non-centrality parameter $\lambda$ following: $\lambda+7=\Delta \chi^2$.

%\TODO{[In light of Fig.~\ref{fig:gaiaDetectability} showing $\Delta \chi^2 > 100$ for periods sometimes tens or hundreds of years I suggest we check that the $\Delta \chi^2$ threshold for $10\%$ correct recovery of parameters (especially eccentricity) is larger than the adopted 100 when P>mission duration. Clearly a 5=parameter model is not a correct reference to compare to (accelerated model would be better, TO BE DISCUSSED). We can test with the Matlab software of Lennart, but I did not do it yet. This should also be fixed in case we plan to release the sensitivity data as I suggested earlier in the text.]}.


\subsection{\EDIT{Radial velocity detection criterion} \label{sec:gaiaDetectMethodRv}} 
% MACP: this para moved from Section1
For a circular orbit, the radial velocity signal is given by \cite[e.g.][Eq.~2.28]{2018exha.book.....P}
\begin{equation}
    K = \sin{i}\ 
\left( \frac{M_p}{M_{*}} \right)
\left( \frac{1~\text{AU}}{a}\right)^{1/2} 
\left( \frac{M_*}{M_\odot} \right)^{7/6}
28.4 \text{ m\,s$^{-1}$}		\ .
\end{equation}
\EDIT{This signal scales as $a^{-1/2}$, i.e., decreasing for wider orbits. The radial velocity signal has no direct dependence on distance, apart from the photometric precision which will depend on the apparent magnitude of the star. We note that inclination cannot be deduced from one-dimensional radial velocity data alone, while it can be derived from (2-dimensional sampled) astrometric data.}

\EDIT{The Radial Velocity Spectrometer (RVS) instrument on-board \gaia \citep{2018A&A...616A...5C, 2019A&A...622A.205K} records a spectrum of every transiting object with $G\lessapprox17$ when the source transits any of rows 4--7 in the field of view (FoV). As there are 7~rows of CCDs in the focal plane, this means that on average 4 out of 7 field-of-view transits will have RVS measurements (Fig.~\ref{fig:FovNumObs}). For the majority of sources the accumulated RVS spectra will be stacked to boost the signal-to-noise and derive an averaged radial velocity. However, for $G_{\text{RVS}}\lessapprox12$ the signal-to-noise ratio will allow the derivation of meaningful radial velocities for each transit, and hence will allow detailed transit-by-transit modelling and the search for velocity variations due to a companion.
The per-FoV radial velocity (RV) precision is of the order of 1\,km\,s$^{-1}$ for the bright stars (Appendix~\ref{sec:gaiaErrorRv}). Despite this being only comparable to the amplitude signal of a $90^\circ$ inclined BD with $80M_\text{Jup}$ mass orbiting at a Jupiter distance from its host star,
with an average of $\sim40$ transits over a 5-year mission it will nonetheless provide orbital constraints on the more massive BDs accompanying bright host stars. 
}

\EDIT{
To explore the detectability of BD using \textit{only} \gaia radial velocities, we derive the approximate per-transit precision in Appendix~\ref{sec:gaiaErrorRv}, 
and compute a $\Delta \chi^2$ criteria for the same levels (30, 50, and 100) as adopted for the astrometric detections. 
For the radial velocity time series of stars with $G_{\text{RVS}}<12$ we compute $\Delta \chi^2 = \chi^2_{\mathrm{min}}\hbox{(1 param)} - \chi^2_{\mathrm{min}}\hbox{(6 parameter)}$, i.e., the difference in $\chi^2$ between a constant radial velocity model fit to the observations (having 1 parameter) and a radial velocity orbital fit to the observations (having 6 parameters). In radial velocity fitting, of the 7 Keplerian parameters the $\Omega$ cannot be determined, and the two components of $a_{*}\sin i$ cannot be separated, hence effectively 5 parameters are left, plus one for the system's systemic velocity. The difference in number of parameters is thus 5 (6--1) and we therefore compute the (noiseless) $\Delta \chi^2=\lambda+5$ for the radial velocity non-centrality parameter $\lambda$ for the threshold levels 25, 45, and 95 to represent the 30, 50, and 100 $\Delta \chi^2$ criteria. The non-centrality parameter in this case is simply the weighted mean of the noiseless observations that include the radial velocity signal of the orbital motion.
}

%[REFERENCE SUMMER DETECTION GAIA PAPER]


\subsection{\EDIT{Transit detection criterion}
\label{sec:gaiaDetectMethodTransit}} 
%\cite{2012ApJ...753L...1D,2010ASPC..430...45S}
%\EDIT{To decide if a transiting BD is detectable we adopt the photometric transit signal-to-noise ratio (S/N) mentioned in Eq.~10 of \cite{2012ApJ...753L...1D}: 
%\begin{equation}\label{eq:transitSn}
%  S/N = \sqrt{n_\text{tr}}\frac{d_\text{tr}}{\sigma(m)} \quad \text{with} \quad d_\text{tr}=\left(R_\text{BD}/R_{*}\right)^2
%\end{equation}
%The photometric sigma $\sigma(m)$ is a function of the observed magnitude $m$ and the error model we derived for the G-band is provided in Appendix~\ref{sec:gaiaErrorPhot}. 
%\cite{2012ApJ...753L...1D} were mainly concerned with identifying periodic signals (hence needing a minimum of at least 3 points in transit) and thus did not really use the S/N criterion in their detection statistics. However, our goal is to simply provide the approximate count of host stars with (potential) detectable DB transits, and thus even a single transit would be sufficient, when the S/N ration is high enough. 
\EDIT{To decide whether a photometric transit is detectable within the photometric time series, we adopt a simple signal-to-noise criterion in which we require each `detectable' transit to have at least a signal to noise of 3
\begin{equation}\label{eq:transitSn}
  S/N = 1.086\frac{ \left(R_\text{BD}/R_{*}\right)^2}{\sigma(G)}	\ .
\end{equation}
The photometric uncertainty $\sigma(G)$ [mag] depends on the observed $G$-band magnitude, and is provided in Appendix~\ref{sec:gaiaErrorPhot}. 
Note that this detection criterion differs from that adopted by \cite{2012ApJ...753L...1D}, where their objective was to identify previously unknown periodic signals, which required a minimum of 3~points in transit. In contrast, our goal is only to estimate the number of host stars with potentially detectable brown dwarf transits, for which even a single well-defined transit would be sufficient. It turns out that the majority of stars will have only 1 or 2 such transits, which must therefore be well-detectable.

% MACP: I suggest deleting this footnote
\gaia has three photometric bands: the broad band $G$ magnitude characterising the main astrometric field, and the two narrower photometric bands $G_\text{BP}$ and $G_\text{RP}$. All bands can potentially detect astrometric eclipses, %\footnote{\EDIT{Gaia image of the week 9 Feb 2017 by Zucker et al.:\newline \url{https://www.cosmos.esa.int/web/gaia/iow_20170209}}}, 
although here we will only consider the most precise $G$-band observations. 

Our simulations do not require us to {\it search\/} for potential transits. Instead, we rigorously compute for each observation whether it is transiting, or partially transiting. We have
}
\begin{eqnarray}\label{eq:transitEq}
      \Delta^\text{*}_{\alpha_*} (t) \text{ [mas]} &=& B  X(t) + G  Y(t) \nonumber \\
      \Delta^\text{*}_{\delta} (t) \text{ [mas]} &=& A  X(t) + F  Y(t)  \nonumber \\
          \Delta^\text{*} (t) \text{ [mas]} &=& \sqrt{ \left( \Delta^\text{*}_{\alpha_*} (t) \right)^2 + \left(\Delta^\text{*}_{\delta} (t) \right)^2 } \nonumber \\
 %    d_\text{*} (t) \text{ [mas]} &=& \sqrt{ \left( B  X(t) + G  Y(t) \right)^2 + \left(A  X(t) + F  Y(t) \right)^2 } \nonumber \\
	%d^\text{*,bd} (t) \text{[au]} &=& (1 + 1/q) \ d_\text{*} / \varpi \nonumber \\
	d(t) \ \text{[au]} &=& (1 + 1/q) \ \Delta^\text{*} (t) \ /  \ \varpi \nonumber \\
	\text{in transit} &=&\begin{cases}
   \text{full transit:} & d(t)< R_\odot - R_\mathrm{BD} \\
    \text{partial transit:} &d(t)< R_\odot + R_\mathrm{BD} 
     \end{cases} \nonumber \\
     \theta_T &=& \text{atan2}(Y,X) \nonumber \\
     z_\text{sign}     & =& \text{sign}(\  \sin( \theta_T + \omega  ) \sin( i) \ ) \nonumber \\
     	\text{transit} &=&\begin{cases}
   \text{primary:} & z_\text{sign} = 1 \\
    \text{secondary:} & z_\text{sign}= -1
     \end{cases}
\end{eqnarray}
where $A,B,F,G$ are the Thiele--Innes orbital parameters in [mas], and $X(t)$ and $Y(t)$ the solution to the Kepler equation at observation time $t$.
The $\Delta^\text{*}_{\alpha_*} (t)$ and $\Delta^\text{*}_{\delta} (t)$ are the time-dependent sky-projected barycentric offsets of the host star in $\alpha$ and $\delta$, respectively.
% MACP: I suggest deleting this next footnote, it adds little
The $\Delta^\text{*}(t)$ is the total sky-projected barycentric offset of the host star in mas, which can be converted into the sky-projected distance\footnote{Note that \EDIT{this expression can only be used for the in-transit computation} of a single companion.} $d(t)$  in au between the host star and the BD companion using the mass ratio $q$ and parallax $\varpi$ in mas. To yield a detectable transit signal, we will only consider the primary transits (where the BD passes in front of the host star, i.e., the host is `behind' the system barycentre as seen from \gaia) corresponding to $z_\text{sign}=1$ in Eq.~\ref{eq:transitEq}, which is computed from the true anomaly $\theta_T$, longitude of periastron $\omega$, and inclination~$i$.


The transit counts provided in this paper include all partial and full primary transits, and assuming $R_\mathrm{BD}=R_\text{J}$ for all simulated BD masses. \EDIT{For completeness we note that  Eq.~\ref{eq:transitSn} overestimates the signal-to-noise for partial transits, as well as for transits close to the outer rim of the stellar disk, as it does not take into account any limb-darkening effects. We ignore these second-order effects as they only affect a small fraction of the data, and will not drastically alter our results.
The $R_\odot$ for each host star is given for the Besan\c con model simulation data ($G>10.5$, see Appendix~\ref{appendix:besancon}) and estimated from the \gaia DR2 data ($G<10.5$, see Appendix~\ref{appendix:gaiaGt10p5})}.






==> figures/Sec_HostStarDistribution.tex <==
%\subsection{Besan\c con model \label{sec:besancon}}

\begin{figure}[!htp]
%  \vspace{0cm}\\
   \centerline{\includegraphics[width=0.49\textwidth]{figures/BSC-B_skyDensity_full_smallb.pdf} }
 %  \centerline{\includegraphics[width=0.49\textwidth]{figures/BscHistMag.pdf} } % without Gaia
   \centerline{\includegraphics[width=0.49\textwidth]{figures/Gaia2BscHistMag.pdf} } % including Gaia
              \vspace{-0.1cm}
%    \centerline{ \includegraphics[width=0.49\textwidth]{figures/BscTypeHist.pdf} }
    \centerline{ \includegraphics[width=0.49\textwidth]{figures/Gaia2BscTypeHistBpRp.pdf} } % including Gaia
    
           \vspace{-0.1cm}
     \centerline{  \includegraphics[width=0.49\textwidth]{figures/BscTeffVsMassMbol.pdf} }
       \vspace{-0.2cm}
\caption{\EDIT{Distribution of the 130~million simulated FGK main sequence (MS) and sub-giants (SG) host stars with $G<17.5$. Top: logarithmic Galactic sky density of the Besan\c con data only, second: histogram of $G$-band counts (bin size: 0.5 mag), third:  histogram of colour (bin size: 0.1) and type (bin size: 0.2), bottom: colour-absolute magnitude diagram for the Besan\c con data only. %\TODO{[add \% to F,G,K stellar type headers.]}
}}
\label{fig:bscFig1}
\end{figure} 


The number of host stars observed by \gaia as a function of stellar parameter is given by our function $N_\text{obs}(\vec{\theta}_*)$. This is taken from the Besan\c con population synthesis model \citep{2003A&A...409..523R, 2012A&A...538A.106R,2014A&A...569A..13R} \EDIT{for stars with $G>10.5$, and is derived from \gaia DR2 data for $G<10.5$, as described in Appendices~\ref{appendix:besancon} and \ref{appendix:gaiaGt10p5}, respectively. The total number of stars brighter than $G=17.5$\,mag is 130~million.
Fig.~\ref{fig:bscFig1} summarises the adopted distribution of host stars, both on the sky, as a function of colour and stellar type, and according to their position in the HR-diagram.
The sky distribution of the \gaia data is not shown, but varies between roughly 2--6 stars per square degree, with the densest regions in the Galactic plane.


Given the adopted constant 0.6\% occurrence rate of BDs around any FGK star (Sect.~\ref{sec:bdFractHostStars}) we can simulate BD systems for a random sample of the 130 million Besan\c con \EDIT{and \gaia DR2 stars and scale the resulting counts. For the main results we simulated a 1\% random sample (1.4 million BD systems), scaled by 0.6 to produce the BD counts used to compute the statistics for the first four rows of result Table~\ref{tab:simResults}. For the $G_{\text{RVS}}<12$ selection (see Sect.~\ref{sect:resultsRv}) we simulated BD systems on the full set of main sequence and sub-giant stars (in our model 1.9~million), and then scaled the simulation counts by 0.006 to get a detailed estimate of the detection rate.}



Throughout this paper we have made the assumption that all \gaia and Besan\c con (host) stars are not in a binary system, apart from the unseen BD component we  simulate. The rigorous inclusion of binarity will most likely reduce the number of detectable BDs, as it complicates the modelling. Also, the BD orbital parameter distributions adopted in this paper are likely to be quite different for those orbiting a binary host system.
} 









==> figures/Sec_Introduction.tex <==

%\TODO{[Introduction on importance and use of brown dwarfs [not yet done]. Motivate FGK selection and magnitude cut. Perhaps add diagrams in paper showing the sensitivity of Gaia to BD of certain mass as function of distance for a given host-star and average sky position.]}

%\subsubsection*{Brown dwarfs}

%- Mention we include high mass planet distribution.
%- mention that ecc of Mjup>10 is roughly consistent with that of above the BD desert
%- for the additional of BD desert filling:
%Grieves2017:
%Ma & Ge (2014) collected data from literature about currently known BD candidate companions around FGK-type stars. While examining the period?mass distribution of BDs, they found a statis- tically significant gap in the short period (P < 100 d) and medium- mass region (35 MJup < MBD < 55 MJup), which they deemed the ?driest? part of the BD desert and likely to be real as it is unlikely caused by detection sensitivity (RV precision) or observation biases (due to survey incompleteness). Three of our new BD candidates, however, are within this driest part of the desert. Fig. 8 shows the Msin i versus period plot of Ma & Ge (2014), but now with candi- dates from table 7 of Wilson et al. (2016) combined with our new MARVELS candidates.


Brown dwarf companions with orbital period $\lesssim10$\,yr are within the range of sensitivity and time-span of various long-running radial velocity surveys 
%2016ASSL..428....3H,        % Hatzes        The radial velocity method for the detection of exoplanets
%2018ASSP...49..199D,        % Diaz        Modelling light and velocity curves of exoplanet hosts
%2018ASSP...49..181F,        % Figuera        Deriving high-precision radial velocities
%2018ASSP...49..239O        % Oshagh        Noise sources in photometry and radial velocities
\citep[e.g.][]{2016ASSL..428....3H,2018ASSP...49..199D,2018ASSP...49..181F,2018ASSP...49..239O}. But despite the many thousands of stars surveyed to date, less than a hundred brown dwarf companions around solar-type stars are currently known \cite[e.g.][]{2014MNRAS.439.2781M,Grieves:2017aa}.
%\TODO{[Check, add various references?]}. 
This has reinforced the evidence for a `brown dwarf desert', i.e.\ the general absence of companions in the mass range $10-80M_\text{J}$, being most pronounced between $30-55M_\text{J}$ \citep{Marcy:2000ab, Grether:2006aa}. 

The low-mass BD distribution seems to be the high-mass tail of the planetary distribution function \citep[e.g.][]{Sahlmann:2011yq}, while the high mass BD distribution seems to be the low-mass tail of the stellar binary distribution function \citep[][Sect.~2.7.1]{1991A&A...248..485D,1992A&A...256..121T,2018exha.book.....P}. This points to formation scenarios that populate the adopted BD mass range having diminishing efficiency toward the BD desert 
\citep{Grether:2006aa,2010A&A...509A.103S,Sahlmann:2011yq,2014MNRAS.439.2781M,2014prpl.conf..619C,2016A&A...585A..46B,2016A&A...587A..64S,2016AJ....151...85T,2016A&A...588A.144W,2017A&A...599A..57B,Grieves:2017aa}. 
%However, the low number statistics of the current BD sample often leads to inconclusive evidence of different populations   \TODO{if we keep sentence we need to back this up with some references}].
 \cite{Sahlmann:2011yq} provide an upper limit on the occurrence rate of tight-orbit ($P\lesssim300$\,d) BD companions around solar-type stars of 0.3--0.6\%, illustrating that to significantly increase the statistics of BDs, one needs to survey millions of host stars.
 

%\subsubsection*{The promise of \gaia} 
So far, the ongoing \gaia ESA mission \citep{2016A&A...595A...1G} has provided the scientific community with \EDIT{three} data releases \citep{2016A&A...595A...2G,2018A&A...616A...1G, 2020arXiv201201533G} containing information on over a billion sources on the sky based on data spanning 13, 22, \EDIT{and 33} months of data, respectively. 
For all sources \gaia measures (near) simultaneously the astrometric position, three-band (spectro)photometry, and radial velocities \cite[for $G_{\text{RVS}}\leq16$~mag][]{Sartoretti2018aa}\footnote{Note that epoch radial velocities will only be published for sources with $G_{\text{RVS}}\leq12-13$~mag, for fainter sources only mean radial velocities will be published.}. \EDIT{For the nominal five-year mission this averages to about about 70 epochs, increasing linearly with time during its extended mission}. 

\EDIT{		% MACP
These three measurements in principle provide three distinct discovery methods for any orbital companions to main-sequence stars, with the astrometric and radial velocity measurements probing the dynamical reflex motion of the host star, and the photometric measurements yielding transit information. We will consider detection yields from these approaches separately, and also in combination.
}

The estimation of orbital parameters of astrometric BDs by \gaia is roughly limited to companions with orbital periods less than the mission length, thus a possible extension providing up to ten years of \gaia data would be greatly beneficial.

% MACP: you refer to upcoming DR3, this should now be re-written?

% \TODO{[perhaps not emphasise this as the sensitivity plots are probably not valid beyond 4-5 yr? To be checked.]}
% will not be able to go much beyond current radial velocity survey period constraints due to its 5-year nominal mission and possible 5-year extension, but because \gaia will  be observing a near-magnitude-complete sample of stars up till around $G$ magnitude 18--19 \TODO{[check, add ref to Gaia paper, and if all previous statements hold water]}, together with it's exquisite astrometric precision, BDs should be found in great number.
\EDIT{No orbital solutions have yet been published by the \gaia consortium; the first of these are expected to be part of the upcoming DR3 release based on 33~months of data. In that release some radial velocity orbital solutions are also expected to be included, though no radial velocity nor astrometric time series will be provided; these will become available with DR4. Although photometric time series have been released for a 550\,000 sample of variable stars in DR2 \citep{2018A&A...618A..30H}, none of these were targeted to photometric transits of unseen companions.}
%So far, astrometric solutions for non-single systems, like the BD companions discussed here, have not yet been published in the first two \gaia data released because of the following reasons: (1)~the presence of (unseen) companions increases complexity of the astrometric signal, demanding a sufficient number of observations and a time baseline comparable to the orbital period(s) to disentangle and characterise a system, (2) noise modelling and instrument calibration needs to have reached a level that allows for accurate signal and uncertainty estimation of individual observations. 


Release of these orbital and time series data will have a major impact on the brown dwarf field, as it will provide a nearly magnitude-complete survey of host stars to at least $G=18$ \citep[DR2,][]{2018A&A...616A..17A}, although extending to a limiting magnitude of $G<20.7$\,mag. As we will show, and largely as a result of \gaia's unprecedented astrometric precision, BDs should be found in large numbers.

Only \EDIT{a few} previous publications have made any estimate of the number of brown dwarfs discoverable by \gaia. \cite{Bouchy:2014aa} estimated a number of 20\,000 BD companions for $G_{\text{RVS}}\leq12$ having both \gaia radial velocity and astrometric measurements.
\EDIT{\cite{2014MmSAI..85..643S} estimated at least several thousands BD companions to $G=16$\,mag extrapolating from known radial velocity samples}.
%, by taking the 3.4 million predicted main-sequence and subgiants with (\gaia band) $G\leq12$ from \cite{Robin:2012aa} and assuming a BD occurrence rate of 0.6\%, and a 100\% detection rate for this sample.,
\citet[][Sect.~2.10.5]{2018exha.book.....P} considered that `\ldots many tens of thousands of [brown dwarf] desert occupants might be expected'. \EDIT{The prediction of several tens of BDs mentioned in \cite{2019ApJ...886...68A} was mainly related to their goal of tightly constraining the mass function, which requires more signal than that for a detection or even an orbital fit. They also examined predictions of unseen companions using simulated \gaia radial velocities.  
 
 In this paper we will not address the issue of \textit{direct} detection of isolated brown dwarfs by \gaia, for which \cite{2014arXiv1404.3896D} predicted `several thousand' with measured parallax. Estimates from DR2 data can be found in \cite{2018ApJ...868...44F}.}

This paper \EDIT{provides up-to-date estimates of the number of brown dwarf companions around FGK host stars expected to be detected in the \gaia astrometric, radial velocity, and photometric transit data. These numbers are derived for the nominal \mbox{5-year} mission (approximately corresponding to DR4), and for an extended 10-yr mission.} 
We limit our analysis to FGK main sequence and sub-giant host stars because only for this restricted population are meaningful occurrence rates, required for our analysis, currently known.

We base our study on the latest \gaia scanning law and instrument models. We derive brown dwarf population distributions, a necessary input to our simulations, from the literature. We then use the Besan\c con population synthesis model as a proxy of the \gaia observed FGK host star distribution, although for the lower and higher mass ends of the stellar mass function \gaia will eventually \textit{define} the observational distribution.

In this paper we will use the term `brown dwarf' to specify a stellar companion in the range $10-80M_{\text{J}}$, despite its overlap with the giant-\text{planet} regime, and without any assumptions on composition or consideration of deuterium burning \citep[e.g.][]{2014prpl.conf..619C}.  We assume that the brown dwarf is sufficiently faint that its light does not influence the astrometric measurement of its FGK-type host star\EDIT{, nor is it considered to be visible in the spectral lines (i.e.\ not a spectroscopic binary). }

Sect.~\ref{sec:gaiaSensitivity} provides an overview of the adopted \gaia detection criteria for astrometric, radial velocity, and photometric transits.  In Sect.~\ref{sec:method} we outline our method of simulating the expected number of brown dwarfs observed by \gaia. The predicted BD numbers and distributions are presented in Sect.~\ref{sec:results}, with discussion of the results in Sect.~\ref{sec:discussion}. Sect.~\ref{sec:conclusions} summarises our conclusions. 

% MACP: I could not see what you refer to with \ref{sec:responseFunctionResults}... Appendix~E is \ref{sec:cdfMass}
Appendices~\ref{sec:gaiaError}, \ref{sec:gaiaErrorRv}, and \ref{sec:gaiaErrorPhot} contain details of the derived error models. Details of the \gaia astrometric response curves are given in Appendix~\ref{sec:responseFunctionResults}. Details of how the data samples were prepared from both the Besan\c con and \gaia DR2 data are given in Appendices~\ref{appendix:besancon} and~\ref{appendix:gaiaGt10p5}.



==> figures/Sec_Method.tex <==
%\begin{equation}
%N_{*,\text{obs}}=N_* \int_{\vec{\theta}_*} f_\text{obs}(\vec{\theta}_*)p_*(\theta_*)\,\text{d}\vec{\theta}_*
%\end{equation}
The number of \gaia detectable BDs can be estimated as

\begin{eqnarray}\label{eq:LL1}
N_\text{det}&=&N_* \int \text{d}\vec{\theta}_* \int \text{d}\vec{\theta}_\text{BD}\,  \nonumber \\
&& f_\text{obs}(\vec{\theta}_*) f_\text{BD}(\vec{\theta}_*) 
f_\text{det}(\vec{\theta}_\text{BD},\vec{\theta}_*) 
p_*(\vec{\theta}_*) p_\text{BD}(\vec{\theta}_\text{BD}|\vec{\theta}_*)
\end{eqnarray}
with the following dependencies:
\begin{itemize}
\item  $N_{\mathrm{*}}$ is the number of F, G, and K (main sequence and subgiant) host stars in our Galaxy;
\item $f_\text{obs}(\vec{\theta}_*)$ is the fraction of observable host stars with stellar parameters $\vec{\theta}_*$;
\item  $f_{\mathrm{BD}}(\vec{\theta}_{\mathrm{*}})$ is the fraction of BDs as function of host star stellar parameters $\vec{\theta}_{\mathrm{*}}$, see Sect.~\ref{sec:bdFractHostStars};
\item $f_{\mathrm{det}}(\vec{\theta}_\text{BD},\vec{\theta}_*)$ is the fraction of detectable BDs by \gaia for a host star with parameters $\vec{\theta}_{\mathrm{*}}$ and BD  parameters $\vec{\theta}_{\mathrm{BD}}$, we will assume in this paper that all systems with $\Delta \chi^2>30$, 50, and 100 are \textit{detected} to the degree as defined in Sect.~\ref{sec:gaiaSensitivity};
\item $p_*(\vec{\theta}_*)$ is the (true) prior normalised probability density function of host stars;
\item  $p_\text{BD}(\vec{\theta}_\text{BD}|\vec{\theta}_*)$ is the (true) prior normalised probability density function of BDs given certain host star stellar parameters $\vec{\theta}_{\mathrm{*}}$, see Sect.~\ref{sec:bdFractHostStars}.
\end{itemize}
Note that the  $f$ fractions % $f_\text{obs}(\vec{\theta}_*)$ and $f_{\mathrm{BD}}(\vec{\theta}_{\mathrm{*}})$ 
are not normalised, and correspond to a number typically much smaller than one when integrated over. 

We use the Besan\c con model \EDIT{and \gaia DR2 data} (see Sect.~\ref{sec:hostStarDistribution}) to predict the number of stars observed by \gaia per stellar parameter (of which stellar type, $G$-band magnitude, and sky position are the most relevant)
\begin{equation}\label{eq:LL2}
N_\text{obs}(\vec{\theta}_*)=N_* f_\text{obs}(\vec{\theta}_*) p_*(\vec{\theta}_*)		\ ,
\end{equation}
reducing Eq.~\ref{eq:LL1} into:
\begin{equation}\label{eq:LL3}
N_\text{det}=\int \text{d}\vec{\theta}_* \int \text{d}\vec{\theta}_\text{BD}\, \
N_\text{obs}(\vec{\theta}_*) f_\text{BD}(\vec{\theta}_*)
f_\text{det}(\vec{\theta}_\text{BD},\vec{\theta}_*) 
p_\text{BD}(\vec{\theta}_\text{BD}|\vec{\theta}_*)
\end{equation}
%
The following sections define the various components in detail, and summarised as follows:
\begin{itemize}
\item Sect.~\ref{sec:bdFractHostStars} introduces the assumption of a constant BD fraction, i.e., $f_\text{BD}(\vec{\theta}_*)=f_\text{BD}$ (= 0.6\%);
\item Sect.~\ref{sec:bdPriors} justifies our assumption that the distribution of BD parameters can be taken to be independent of the stellar parameters, i.e.\ 
$p_\text{BD}(\vec{\theta}_\text{BD}|\vec{\theta}_*)=p_\text{BD}(\vec{\theta}_\text{BD})$, and then goes on to specify that distribution; 
\item finally Sect.~\ref{sec:hostStarDistribution} gives $N_\text{obs}(\vec{\theta}_*)$ from the Besan\c con model.

\end{itemize}


 


\subsection{BD fraction as a function of host stellar parameters\label{sec:bdFractHostStars}} 
Estimates of the numbers of BD detectable with \gaia rest on the presently known occurrence rates as function of host star and companion properties.
For the CORALIE planet search sample containing 1600 Sun-like stars within 50 pc, \cite{Sahlmann:2011yq} derived a range of 0.3--0.6\% for the frequency of close-in brown-dwarf ($P\lesssim300$\,d), which is consistent with the $<0.5\%$ upper limit of \cite{Marcy:2000ab}, and the recent 0.56\% for $P\lesssim300$\,d of \cite{Grieves:2017aa}. \cite{Grether:2006aa} find a similar occurrence rate of  $<1\%$ when considering BD companions around solar-type stars with periods $P\lesssim5$\,yr.

For AF-type main sequence stars, \citet[][Table 4]{Borgniet:2017aa} found that for the lower mass sample ($M_{*} \leq 1.5 M_{\odot}$, i.e., F-type stars) the occurrence rate of BDs with $1<P<1000$~d is $\leq 2\%$ (similar for both $1<P<100$~d and $1<P<10$\,d), though with a $1\sigma$ confidence interval between 0--7\%, hence consistent with, but not more constraining than, the previously mentioned occurrence rates. \EDIT{At the lower end, \cite{2016A&A...587A..64S} found a rate of $0.29\pm0.17\%$ for BD having a Kepler transit with $P<400$\,d \cite{2010Sci...327..977B}, while at the high end \cite{2016MNRAS.458.3272K} used SOPHIE to study FGK stars within 60~pc in the northern hemisphere, finding
12 new BD, and concluding a BD rate of $2.0 \pm 0.5 \%$ for $P<10\,000$\,d. The latter is likely overestimated due to its derivation from RV-data.}

\cite{Sahlmann:2011yq} conclude that the CORALIE sample was too small to make any inferences on a dependence on the metallicity distribution of the host stars, as found for planet host stars \citep[e.g.][]{Santos:2001aa}.

We therefore adopt a constant BD fraction for this study, i.e., $f_\text{BD}(\vec{\theta}_*)=f_\text{BD} = %0.3-0.6\%$,  0.3 -- 0.9
0.6\pm0.3 \%$, where the lower value is based on the lower estimate of $0.3\%$ by \cite{Sahlmann:2011yq} for $P\lesssim300$\,d \EDIT{and consistent with \cite{2016A&A...587A..64S}}, and the upper value of $0.9\%$ by the upper limit of $1\%$ from \cite{Grether:2006aa} for $P\lesssim5$\,yr. Though this 50\% uncertainty will dominate the accuracy of our estimate of the number of expected BD discoverable, it is the most realistic value to use given the current data available. We will limit the longest simulated periods to 5\,yr, as discussed in the following section.



\subsection{BD prior orbital parameters for simulations \label{sec:bdPriors}} 
%\TODO{[TODO]}
%A study on AF-type main sequence stars of \cite{Borgniet:2017aa} finds the that the frequency of BDs the 1 -10$^3$~d is consistent with the "brown dwarf desert".
%the paucity of BD-mass companions compared to both GP and low-mass stellar companions at SMA below 3--5 au) reported around solar- like FGK dwarfs by transit and RV surveys (with a $<1\%$ fre- quency, see, for example, Grether \& liuneweaver 2006


\paragraph{Mass distribution}
As discussed in the introduction, there is clear evidence for a general absence of sub-stellar companions in the BD mass range (the so-called BD `desert'), being most pronounced between $ 30-55M_{\text{J}}$. Examining the cumulative mass distribution function from Fig.~18 of \cite{Sahlmann:2011yq} and Fig.~3 of \cite{2014MNRAS.439.2781M}, it appears that about half of the BD candidates reside on one side of this desert. Given their paucity, the relative occurrence rate as a function of mass is currently rather ill-constrained.
%it is currently not possible to define a precise function that provides the relative occurrence rate as function of mass. 
Adopting the power-law fits of \cite{Grether:2006aa}, as shown in their Figs~8 or 9, would result in zero BDs between 13--55 or 20--57 $M_{\text{J}}$, respectively, which seems too restrictive as a generative function for this study in which we focus on the $10-80M_{\text{J}}$ range.

Based on the above, we therefore create a customised mass distribution function suited for this study:
\begin{itemize}
\item all companions have masses in the range $10-80M_{\text{J}}$,
\item the BD `desert' occurs at half the cumulative mass distribution \citep[conforming to Fig.~18 of][]{Sahlmann:2011yq},
\item we assume a linear relation in $\log_{10}(M_{\text{BD}})$ \citep[as in][]{Grether:2006aa} on both sides of the desert: one with a negative slope between $10-30M_\text{J}$ and one with a positive slope between $55-80M_{\text{J}}$.
\item we add a constant level in $\log_{10}(M_{\text{BD}})$ of $2\%$ of the BD companions in the $30-55M_{\text{J}}$ range, which is a rate that could easily lead to non-detection in the previous studies given their sample sizes.
\end{itemize}
The result is shown in Fig.~\ref{fig:hollMassFunction}. The cumulative density function is given in quadratic form $c + bx + ax^2$, with $x=\log_{10}(M_\text{J})$:
\begin{equation}
%{\displaystyle%\scriptstyle % \textstyle
% incorrect: linear in CDF:
%  CDF_M(x)=\begin{cases}
%    -1.027 + 1.027 x, & \text{$10\leq M_\text{J} <30$} \\
%   \ \ \ 0.378 + 0.076 x, & \text{$30\leq M_\text{J} <55$}\\
%    \ \  -4.73  + 3.01x, & \text{$55\leq M_\text{J} \leq 80$}
%  \end{cases}
    {\rm CDF}_M(x)=\begin{cases}
    -3.974 + 5.969x -1.995x^2, & \text{$10\leq M_\text{J} <30$} \\
   0.3778 + 0.0760x, & \text{$30\leq M_\text{J} <55$}\\
    55.052 -62.753x + 18.05x^2, & \text{$55\leq M_\text{J} \leq 80$}
    \label{eq:massDCF}
  \end{cases}
\end{equation}
The normalized histogram values shown in Fig.~\ref{fig:hollMassFunction} are simply the first derivative of CDF$_M(x)$.
In the simulations the BD mass $(M_{\text{BD}})$ was generated as a random number using the inverse CDF (Appendix~\ref{sec:cdfMass}).
\begin{figure}[h]
%  \vspace{0cm}\\
  \includegraphics[width=0.5\textwidth]{figures/Holl19_BDmass_hist_cdf.pdf} 
 \caption{Adopted BD mass distribution in this study, see text for details.
}
\label{fig:hollMassFunction}
\end{figure} 


\paragraph{Period distribution}
Though radial velocity and transit observations are biassed towards the detection of short-period objects, observations show that the number of BDs increases with orbital period, which is consistent with direct imaging surveys \citep{Diaz:2012aa, 2014MNRAS.439.2781M}.  %Because the \gaia response function is highly dependent on period it is essential that we have some good representation of the period distribution. 
Because \gaia 's \EDIT{astrometric} sensitivity increases with increasing period up to the mission duration (Appendix~\ref{sec:gaiaResponseComp}), it is important to have a good representation of the period distribution up to at least the nominal 5~yr mission length. Most literature data have poor statistics beyond several years orbital period (and often limited to only 300--500\,d), so we have limited our adopted period distributions to 5~years.

To satisfy our need to sample beyond more than 1--2~years, we derived the period distribution from the samples of \cite{2014MNRAS.439.2781M} and \cite{Diaz:2012aa} consisting of (partially overlapping) BDs with masses between 9 and 90 $M_\text{J}$ and orbiting solar-type stars with a period shorter than $\sim 10^4$~d. Unfortunately these studies contain an aggregation of identified objects without the kind of bias sample corrections applied in, e.g., \cite{Grether:2006aa},
%\footnote{\TODO{[I could not find the mass and period data used in \cite{Grether:2006aa}, only the generic table 1 data in their paper, or is this easily matched against e.g. some exoplanet database?]}}
Accordingly, their period distributions should probably be used as approximate at best, which is already illustrated by their differences in the cumulative distribution functions (Fig.~\ref{fig:cdfHistPeriodFit}).
Since we need to represent the longest periods most accurately, because they have the highest detectability, we bias our fits towards them. Hereafter these are referred to as the `Ma\,\&\,Ge' and `D\' iaz' fits and labelled `our fit (large $P$)' in Fig.~\ref{fig:cdfHistPeriodFit}. For illustration we also fit the `whole' \cite{Diaz:2012aa} curve with a more complex model (see `D\' iaz our fit (all $P$)' in Fig.~\ref{fig:cdfHistPeriodFit}), though the comparison with the histogram seems to suggest such a model does not seem to really represent the underlying distribution better, and it will not be further used for this study. Because the period distribution is amongst the most important factors in determining our predicted numbers, we will asses (and combine) the result of both the Ma\,\&\,Ge and D\' iaz fits, because they nicely represent two rather different steepnesses of the assumed period distribution towards larger periods.
%\TODO{[add the cdf and inverse cdf functions of Ma\,\&\,Ge and Diaz fits if agreed these two should be used in the paper]}

In both the Ma\,\&\,Ge and D\' iaz fits we set the lower limit to 1\,d, based on the apparent cutoff in the population (as these systems should have a high detectability in the radial velocity studies). The lower panel of Fig.~\ref{fig:cdfHistPeriodFit} suggest that the distributions peak around 2.5--5\,yr, though it is unclear if this could be ascribed to a selection effect in the surveys (due to the survey lengths) or is really a feature of the underlying BD distribution.  In case a significant population exists with $P>5$\,yr, \gaia will be able to detect a large fraction of those with periods at least several years beyond the final \gaia mission length.

\begin{figure}[h]
%  \vspace{0cm}\\
  \includegraphics[width=0.5\textwidth]{figures/MaGe14DiiazRaimbault_period_cumAndHist1_v2.pdf} 
% \includegraphics[width=0.5\textwidth]{figures/MaGe14_period_hist1.pdf} 
\caption{Period distribution of the BD sample from \cite{2014MNRAS.439.2781M} and \cite{Diaz:2012aa} having masses between 9 and 90 $M_\text{J}$ orbiting solar-type stars. % where we applied the 1~d4<P<5~yr cut to the period.  
Top: the cumulative distribution function for  BDs, the `large P' fits of Ma\,\&\,Ge and D\' iaz are used to generate \EDIT{the BD period distributions and will be referred to as $\textrm{P}_\textrm{distr}$=Ma\,\&\,Ge and $\textrm{P}_\textrm{distr}$=D\' iaz, respectively}. The bottom figure shows the log-binned histogram with the corresponding fit-curves (bin size $\log_{10}(1.98)$). Our simulations are limited to the indicated (non-shaded) period range  1\,d\,$<P<$\,5\,yr. The \cite{raimbault19} data is used for an additional bootstrap sample estimate (Sect.~\ref{sec:raimbaultBootstrap}).
}
\label{fig:cdfHistPeriodFit}
\end{figure} 


 %We bin the sample in $\log( P )$ and derive a logarithmic fit: $d N / d (\log P) = 6.4 \log(P)$, and exponential fit: $d N / d ( \log P) = 2 \exp(0.81\ \log(P))$ for periods up to 5 years, as shown in Fig.~\ref{fig:diaz12HistPeriodFit}. The former overestimates the intermediate periods around $10^{1.5} - 10^{2.5}$ and underestimates the long periods, while the latter follows the distribution better and perhaps slightly underestimating the short periods. The input period distribution used in this paper will be drawn from the (normalised) logarithmic fit, though we will check if drawing from the (normalised) exponential fit gives significant different results. We decides to limit the period distributions between 1~d and 5~years. The lower limit is based on the apparent cutoff in the population, and the upper limit based on our poor understanding of the sample beyond this period range (as the drop-off in the sample is mainly due to the limited survey time-span of radial velocity surveys).
%As shown in Sect.~\ref{sec:gaiaResponseComp}, the detectability of \gaia peaks at the mission length, i.e. $\sim 1830$~d or $\sim 3650$~d, for five and ten years, respectively, and thereafter quickly drops off. Hence, cutting the input distribution to 5 year will not impact the simulated results too much (given the  current BD population knowledge), though we would like to point out that in case a significant population exists with periods larger than five years and shorter than several tens of years, \gaia will be able to sample a large part of it.

\paragraph{Period--eccentricity distribution\label{sec:eccVsPeriod}} 

%\cite{Diaz:2012aa} and \cite{2014MNRAS.439.2781M} show that eccentricity generally increases with the BD period. 
%The absence of high eccentricities for very short periods can be attributed to the circularisation effect of tidal interactions
%\cite{2014MNRAS.439.2781M} finds that ``the period-eccentricity distribution of BDs with (minimum) masses greater than 42.5~M$_{\mathrm{J}}$ is consistent with a circularization limit of $\sim12$~d, which is similar to that found in nearby stellar binaries \citep{Raghavan:2010aa}''.
 %\TODO{[this is what I wrote, is this a generally correct statement?]}. 
\cite{2014MNRAS.439.2781M} found that there seems to be a statistically significant different distribution of eccentricities for BDs below and above $42.5M_{\mathrm{J}}$ (the `driest' part of the BD desert). For the BDs with (minimum) mass above $42.5M_{\mathrm{J}}$ they identify the short period distribution to be consistent with a circularisation limit of $\sim$12~d, similar to that of nearby stellar binaries \citep{Raghavan:2010aa}. Also, these massive BDs seem to have an  apparent absence of eccentricities below $e<0.4$ for periods $300<P<3000$~d, while these eccentricities are populated by BDs with (minimum) masses below $42.5M_{\mathrm{J}}$. Additionally, the latter sample suggests a reduction in maximum eccentricity toward higher (minimum) mass, while such trend seems absent for the sample with (minimum) mass above $42.5M_{\mathrm{J}}$.

As for the period distribution, we inspect the eccentricity distribution of \cite{2014MNRAS.439.2781M} and \cite{Diaz:2012aa} in Fig.~\ref{fig:eccDist}. Generally there is not a clear distinction between the lower mass and higher mass regimes in the \cite{2014MNRAS.439.2781M} data, and we simply adopt a single fit that allows us to draw eccentricities in the range 0--1 in a continuous fashion. 
%\TODO{[add the cdf and inverse cdf functions of eccentricity fit show in the figure]}
%
The \cite{Diaz:2012aa} sample has a slightly more eccentric distribution than our fit, though this is in the interval $e=0-0.6$, for which our detection efficiency varies only by about 10\% (Fig.~\ref{fig:gaiaDetecEcc}). Accordingly, if the true brown dwarf eccentricity distribution follows the D\' iaz curve, it would have only a marginal effect on the predictions.  

\cite{Kipping:2013aa} suggested that the orbital eccentricity distribution for extrasolar planets is well described by the Beta distribution. We did not perform an extensive fitting, but for illustration plot the Beta distribution $B(2,4)$ in Fig.~\ref{fig:eccDist}, having the rough mean of the distributions shown (0.30~for  \cite{2014MNRAS.439.2781M}, and 0.41 for \cite{Diaz:2012aa} for $P<5$\,yr). This illustrates that there in no good match with  \cite{2014MNRAS.439.2781M}, although it resembles the \cite{Diaz:2012aa} reasonably well. The good fit found for planetary data, $B(0.867,3.03)$, provides a poor match to these data, heavily under-predicting the observed non-zero eccentricity distribution.

\begin{figure}[h]
%  \vspace{0cm}\\
 \includegraphics[width=0.5\textwidth]{figures/MaGe14DiazRaiimbault_ecc_hist1Cdm.pdf} 
%   \includegraphics[width=0.5\textwidth]{figures/MaGe14_ecc_hist1} 
\caption{Eccentricity distribution of the BD sample from \cite{2014MNRAS.439.2781M} and \cite{Diaz:2012aa}. Top: the cumulative distribution function for  BDs. The `Ma\,\&\,Ge' fit is used for the simulations in this paper. The bottom figure shows the binned histogram with the corresponding fit-curve (bin size 0.05). The \cite{raimbault19} data is used for an additional bootstrap sample estimate (Sect. ~\ref{sec:raimbaultBootstrap}).
}
\label{fig:eccDist}
\end{figure} 

Having chosen our independent distribution functions, we can inspect the period--eccentricity distribution of both \cite{Diaz:2012aa} and \cite{2014MNRAS.439.2781M} in Fig.~\ref{fig:pEcc}. %~\ref{fig:diaz12HistPeriodFit}.
We adopted a circularisation period of $P_{\mathrm{circ}}=10$\,d, using the formulation of \cite{Halbwachs:2005aa}, being an obvious feature in the combined parameter space. We did not adopt a specific mass-dependent eccentricity distribution, in part because the effect is only very marginal in Fig.~\ref{fig:eccDist}), but also because \cite{Grieves:2017aa} find some new candidates (their Fig.~9) which do not follow the regimes introduced by \cite{2014MNRAS.439.2781M}, although they do still support a two-population trend.

The way the samples for our simulations are constructed is by first drawing a period from either the Ma\,\&\,Ge or D\' iaz period-distribution fit. Then we use this period to compute the maximum eccentricity allowed due to the circularisation criterion, and use this to limit the range of the drawing of the eccentricity, effectively cutting the PDF from which we draw the eccentricity, from zero to the maximum eccentricity allowed. This means that the effective eccentricity distribution that is used has an increased rate of low eccentricity systems with respect to the CDF fit-line shown in Fig.~\ref{fig:eccDist}.


% MACP: please review the figure caption because I could not understand it!
\begin{figure}[h]
%  \vspace{0cm}\\
 % \includegraphics[width=0.5\textwidth]{figures/MaGe14_P-Ecc.pdf} 
    \includegraphics[width=0.5\textwidth]{figures/MaGe14Raimbault19_P-Ecc.pdf} 
\caption{Period--eccentricity distribution of the BD sample from \cite{2014MNRAS.439.2781M} split in low-mass and high-mass samples, \cite{Diaz:2012aa}, and from \cite{raimbault19} only the companions in the $10-80M_\text{J}\sin i$ range. A circularisation limit of 10\,d is adopted, hence all objects with $P<10$\,d have $e=0$ in our simulations. We limit (most of) our analyses to companions in the interval 1\,d\,$<P<$\,5\,yr (i.e., between the shaded areas). 
%\TODO{[Align the overlapping points of the two datasets, as the \cite{Diaz:2012aa} were extracted from the plot in their paper...]}
}
\label{fig:pEcc}
\end{figure} 





==> figures/Sec_Results.tex <==
The total number of BDs around \gaia observable host stars is about 780\,000, i.e.\ 0.6\% of the 130~million Besan\c con stars, listed on the top row of Table~\ref{tab:simResults}. To estimate the \textit{detectable} number of BDs we have to adopt the various models discussed in the previous section. The table columns (and figure labels) \EDIT{  $P_\textrm{distr}$\,=\,Ma\,\&\,Ge and $P_\textrm{distr}$\,=\,D\' iaz`} specify the underlying period distribution used in the simulations (see Sect.~\ref{sec:bdPriors} and Fig.~\ref{fig:cdfHistPeriodFit}). 
Because the number of \gaia detections is highly sensitive to the period distribution, and it is amongst the most ill-defined priors, we express the final numbers as the range of the counts resulting from the two models. As seen from Table~\ref{tab:simResults}, the D\' iaz period distribution predicts about 20--30\% more BDs than Ma\,\&\,Ge.
%Table~\ref{tab:simResults} summarises the results of this paper, showing that at the end of the 5-year nominal mission we can expect around 

\EDIT{Table~\ref{tab:simResults} allows us directly to draw some overall conclusions: 
\begin{itemize}
    \item the number of astrometric BDs detectable with \gaia will be in the tens of thousands;
    \item the radial velocity time-series for $G_{\text{RVS}}<12$ will be able to detect thousands of BDs;
    \item the total number of stars with a few photometric detectable BD transits will also be in the thousands;
    \item stars with both good astrometric and radial velocity BD detections will be in the hundreds;
    \item the number of transiting exoplanets in combination with radial velocity detection will be in the tens;
    \item and there will be only several in combination with astrometry;
    \item only a few combined detection in all domains are likely.
\end{itemize}}
% MACP: not worth the effort or space, I suggest
\EDIT{[THIS summary ASKS FOR A NICE VENN DIAGRAM OF THE 3 DOMAINS, I think I should make it...]

The sky distribution of our recovered BDs is shown in the first panel of Fig.~\ref{fig:resultsTypeRelated}, showing that it generally follows the Galactic host-star distribution, `weighted' by the available number of observations shown in the second panel.}

The distribution as a function of stellar type is illustrated in the third panel of Fig.~\ref{fig:resultsTypeRelated}, showing that our recovery peaks with 40\% G-type stars, with about 32\% amongst K-stars, and 28\% around F-stars. The recovery numbers are declining at the edges of our adopted range of stellar types, i.e.\ towards the more massive F-stars and less-massive K-stars, confirming our assumption in the introduction that the majority of BDs detections is expected around FGK-stars. The vast majority of detections (85\%) is around main-sequence stars, with only 15\% coming from the sub-giants.

\EDIT{For the following summaries, the results from Table~\ref{tab:fracTransiting} and \ref{tab:RbsimResults} have also been included.}

\subsection{\EDIT{Detections by astrometry}}
\EDIT{For the adopted BD mass range $10-80M_{\text{J}}$ we conclude that using astrometry alone, \gaia should detect between 41\,000--60\,000 ($\pm$25\,000) BDs, of which 28\,000--42\,000 ($\pm$15\,000) BDs % ($\sim$10--80~M$_{\text{J}}$ ) 
should be reliably detected out to several hundred~pc. The majority will have $P>200$\,d, although extending up to the 5~yr adopted upper period-limit. Good orbital solutions will be possible for about 17\,000--26\,000 ($\pm$10\,000) systems. 

Fig.~\ref{fig:results1page} \EDIT{[not yet updated with Gaia data...]} shows that the distribution peaks around $G\sim14-15$, and that the majority of recoveries are for the more massive BDs. Note that even though we depleted the input distribution of the `desert' region to contain only 2\% of the rest of the BD, there are still tens of confident detections. The detection fraction (completeness) steadily increases towards the bright end, though for the most populated magnitudes it reaches only 20--30\%. For a 10-yr mission, this number rises to 30--40\%. The distance and magnitude limits are also significantly extended for the 10-yr mission.}


\subsection{\EDIT{Detections by radial velocity\label{sect:resultsRv}}}
\EDIT{An interesting sub-sample will be those sources with \gaia radial velocity time series, assumed to be those with $G_{\text{RVS}}<12$ ($G\sim 11.3$). We find that \gaia will be able to detect between 6200--8200 BDs, of which 5300--7200 robustly, and 4300--6000 with good orbital parameters. As shown in Fig.~\ref{fig:results1pageRv}, and as expected, the largest numbers are found at short orbital periods and for the most massive BDs ($55-80M_{\text{J}}$), although several tens of those will extend to the lowest BD masses. 
The largest number of detections is around $G=12$, where the detection fraction is around 30--40\%. A 10-year mission boosts this to 50--60\%.
 
The combination of astrometric and radial velocity detections (i.e. the last three rows of Table~\ref{tab:simResults} and shown in Fig.~\ref{fig:results1pageAstroRv}) yields  1700--2700 systems, of which 450--570 have good orbital solution from either data set. The numbers double for a mission extension of 10~years. This will be an important sample, since a joint solution would better constrain all system parameters. Additionally, since all sources with \gaia RV time-series are relatively bright, this set will be ideal for follow-up observations.
}


\subsection{\EDIT{Detections by photometric transits\label{sec:transit}}}
\EDIT{
For each simulation we list the number of sources that have non-zero detectable transits (S/N\,>\,3) in parenthesis in Tables~\ref{tab:simResults} and \ref{tab:RbsimResults}, together with their average number of observation in transit. The transit depth and period distribution of the Ma\,\&\,Ge 5-year sample are shown in Fig.~\ref{fig:numInTransit}.

As seen from Table~\ref{tab:simResults} detectable photometric transits are expected for some 800--4000 mainly short-period BDs, each yielding 2--4 transits on average.
%, though this number drops to only 35--120 for the bright-star regime ($G_{\text{RVS}}<12$). 
%As seen from Table~\ref{tab:simResults} perpaps 1000-3000 BDs are expected to have each on average 2.5 observable transits in their \gaia photometry, 
This would already dramatically increase the known BD sample through photometric detection alone, although this sample is heavily dominated by BDs having periods within several (tens of) days as seen in Fig.~\ref{fig:numInTransit}. For $G_{\text{RVS}}<12$ this number drops to 35--120 BDs each with typically three observable transits. For astrometrically detectable BDs, the numbers drop to around 10~BDs, each with $\sim2$ observable transits (similar to when we restrict ourselves to $G_{\text{RVS}}<12$). A 10-yr mission would double or triple these small numbers.

Because both detection methods favour large orbital inclination and short orbital period, several tens of systems with radial velocity detections should also display transits.
}

In Table~\ref{tab:fracTransiting} we list the total transit statistics for the Ma\,\&\,Ge simulation for different period bins. For example, for the 256--512~day bin we can see that of all observations of all random oriented sources there is 1 in  81\,000 observations in transit ($1/f^\text{obs}_\text{tr}$), and 1 in 1800 sources that have non-zero transits ($1/f^\text{src}_\text{tr}$). For those sources that have non-zero transit, the mean number of transits is $\langle N^\text{obs}_\text{tr} \rangle=1.8$. %\TODO{[Michael: as validation we should check if the 1 in 1700 of your paper is consistent with this table.]}

The largest main sequence stars\footnote{Using radii from reference in footnote~\ref{footnoteMamajek}.} have diameters around $1.79R_{\odot}$ (F0V) and the smallest around $0.65R_{\odot}$ (K9V). For an adopted BD radius of $R_\text{J}\sim0.1R_{\odot}$, this means that the predicted transit depth $(R_{\mathrm{BD}}/R_*)^2$ ranges between 0.3--2.3\%, corresponding to $\Delta m\simeq3-23$\,mmag. This is around or above the \gaia noise limit for most of the considered magnitude range. In general, due to the low average number of transits per system, it will be difficult to clearly identify BDs from \gaia photometry alone, though a fraction of (mainly short-period) BDs will have sufficient transits to allow for a \gaia photometry-only identification, as shown in the `ALL' selection of the middle panel of Fig.~\ref{fig:numInTransit}. %given the large sample there will be a still rather significant  can exthere will be a fraction that has sufficient transits that will allow for a \gaia photometric-only detection. 
In the marginal astrometric detected cases ($\Delta \chi^2 \sim30$) any detected transits will further help to constrain the orbit.

In the Ma\,\&\,Ge 5-year transit sample, shown in Fig.~\ref{fig:numInTransit}, more than 80\% of the identified transiting systems with astrometric detectability are around main sequence stars. The `ALL' sample consists of 40\% sub-giant stars, of which the radius can extend to $2.5-3R_{\odot}$ and hence can have transit depths as small as 3~mmag.


\begin{figure*}[!htp]
%  \vspace{0cm}\\
  \includegraphics[width=0.98\textwidth]{figures/manyTransitMa14.pdf} 
\caption{\EDIT{Transit statistics from the $\textrm{P}_\textrm{distr}$ Ma\,\&\,Ge simulation for a 5-year and 10-year mission of 1.5~million randomly oriented BDs. These BD number counts are scaled by 0.6 in Table~\ref{tab:simResults} to represent a 0.6\% BD occurence rate, see Sect.~\ref{sec:results}. Detailed period-binned statistics of the `ALL' part are shown in Table~\ref{tab:fracTransiting}. 
}}
\label{fig:numInTransit}
\end{figure*} 




\begin{table}[h]
\caption{Transit statistics from the Ma\,\&\,Ge simulation (for a \mbox{5-yr} mission for `ALL': irrespective of the systems detectability and sky orientation) according to period. Here, 
$f^\text{obs}_\text{tr}$ is the fraction of observations in transit, and 
$f^\text{src}_\text{tr}$ is the fraction of sources having any observations in transit, both being for randomly oriented systems.
For sources that have transits, $\langle N^\text{obs}_\text{tr}\rangle$ is the mean number of transits per source. The numbers in the last two bins are particularly poorly defined due to their low occurrence rates in the simulated data. \EDIT{[did not yet re-do, though probably does not change much]}}. 
\label{tab:fracTransiting}     
\centering                        
\begin{tabular}{c  r r r r}        
\hline\hline      
period bin [day] &  $1/f^\text{obs}_\text{tr}$ & $1/f^\text{src}_\text{tr}$ & $\langle N^\text{obs}_\text{tr} \rangle$  \\
\hline                                             %inserts single line
1--2 & 60 & 4.3 & 5.6 \\
2--4 & 150 & 7.1 & 3.8 \\
4--8 & 350 & 12 & 2.8 \\
8--16 & 900 & 25 & 2.2 \\
16--32 & 2150 & 51 & 1.9 \\
32--64 & 5200 & 115 & 1.7 \\
64--128 & 13\,000 & 270 & 1.6 \\
128--256 & 29\,000 & 625 & 1.7 \\
256--512 & 81\,000 & 1800 & 1.8 \\
\hdashline
512--1024 & 210\,000 & 4900 & 1.9 \\
1024--1826 & 450\,000 & 11\,000 & 1.9 \\
\hline     
\end{tabular}
\end{table}




%---from abstract
%Photometric detectable transits (S/N>3) are expected for some 800--4000 mainly short-period BDs have on average 2--4 transits, though this number drops to only 35--120 for the bright-star regime ($G_{\text{RVS}}<12$). Transits in sources with astrometric detection are rare as these are mainly long-period BDs and thus only a a dozen or so are expected. Transits in combination with radial velocity detections is much more favourable as both have higher gain for short period objects, and hence several tens of these are expected to be found. The number of systems with detections in all three domain will likely be countable on one hand.

%The extension to a 10-year mission is giving a huge boost in all the detection rates: the astrometric detections increase by $\sim 70\%$ ($\sim 25 \%$ for $G_{\text{RVS}}<12$), the radial velocity detections increase by 70--100\%, and the number of transiting BDs by about 300--500\% (250--300\% for $G_{\text{RVS}}<12$) having typically a few more transits per source.





%---- OLD

%Applying this, we predict that \gaia will identify 17\,000--21\,000 BDs with well-determined orbital parameters, 
%which increases to 27\,000--34\,000 when lowering our threshold to reliable detections,
%and reaches around 40\,000--49\,000 when also including just marginal BD detections. For a 10-yr extended mission these numbers increase by roughly a factor of 1.7, also extending further in the fainter magnitude regime, see Figs.~\ref{fig:results1page}, ~\ref{fig:results1pageRv}, and ~\ref{fig:results1pageAstroRv}.

%Figures~\ref{fig:results1page} and \ref{fig:magHist} show they should be detectable out to maximum distances of some 1--1.5\,kpc for the nominal 5~yr \gaia mission, with the majority having periods above 100\,d (up to the 5~yr adopted upper limit). As expected from the astrometric signal dependence, the recovered mass distribution is heavily skewed towards the heavy companions with 85--90\%  having a mass above $40M_{\text{J}}$ while in the input prior this was 50\%.
%The detections per magnitude in Fig.~\ref{fig:magHist} shows that the distribution peaks around $G\sim14$ (top panel), and that the fraction of detected sources is steadily increasing towards the bright end (bottom panel), though only reaching a detection efficiency just above 50\% at $G\simeq10$. The number of BDs that are missing from our estimation due to this simulation host-star magnitude cut is perhaps 1000-1500 (see end of Sect.~\ref{sec:hostStarDistribution}).
%5--10\%, see discussion in Sect.~\ref{sec:missingBrightHost}.



% removed on Alessandro's request
%For completeness we also provide a comparison with the more simplistic SN-criterion in Appendix~\ref{appendix:snCrit}: see Table~\ref{tab:simResultsSnCrit} and Fig.~\ref{fig:snCritComparison}.



\begin{table*}[t]
\caption{Simulation results. The number of detected BDs is tabulated, with in parentheses the number of host stars having \EDIT{individually detectable photometric transits in \gaia data (S/N>3)} together with their mean number of transits. 
The two period distributions ($\textrm{P}_\textrm{distr}$) `Ma\,\&\,Ge'  and `D\' iaz' are detailed in Sect.~\ref{sec:bdPriors} (Fig.~\ref{fig:cdfHistPeriodFit}).
\EDIT{All counts could be up to $50\%$ higher or lower due to the uncertainty on the assumed $0.6\%$ BD occurrence rate (see Sect.~\ref{sec:bdFractHostStars})}.
}. 
\label{tab:simResults}     
\centering    
%\renewcommand{\arraystretch}{1.0}                    
\begin{tabular}{c c c | r @{\ }l r@{\ } l | r@{\ } l  r@{\ } l}          % 
\hline\hline      
Magnitude & Astro & RV & \multicolumn{4}{c|}{5-yr nominal} & \multicolumn{4}{c}{10-yr extended} \\
%\cline{2-5}    
selection & $\Delta \chi^2$ & $\Delta \chi^2$ & \multicolumn{2}{c}{$\text{P}_\text{distr}$ = Ma\,\&\,Ge }   & \multicolumn{2}{c|}{$\text{P}_\text{distr}$ = D\' iaz} & \multicolumn{2}{c}{$\text{P}_\text{distr}$ = Ma\,\&\,Ge }   & \multicolumn{2}{c}{$\text{P}_\text{distr}$ = D\' iaz}  \\    % table heading
\hline                                 
--                 & -- 	        & --	& 780\,000 & (3100: 2.5)     &   780\,000 	&(2000: 2.5)        & 780\,000 &(4000: 4.0) 	& 780\,000 &(2700: 3.7) \\
\hline
--                 & $>30$         & --	    & 41\,000 & ( \ \ \ 16: 2.0)     &   50\,000 & ( \ \ \  15: 1.9)   & 64\,000 & ( \ \ \ 56: 2.0) & 77\,000 & ( \ \ \  43: 1.7)  \\
--                 & $>50$         & --	    & 28\,000 & ( \quad \ 8: 2.1)    &   34\,000 & ( \ \ \  11: 1.9)   & 45\,000 & ( \ \ \ 33: 1.9) & 55\,000 & ( \ \ \  27: 1.8)  \\
--                 & \ \ $>100$    & --	    & 17\,000 & ( \quad  \ 4: 1.9)    &	21\,000 & ( \quad \  4: 2.1)  & 28\,000 & ( \ \ \ 15: 1.9) & 35\,000 & ( \ \ \  18: 1.7)  \\
\hline
\hline
$G_{\text{RVS}}<12$ & -- 		    & --	& 12\,000 & ( \   120: 2.9)      & 12\,000 & ( \ \ \ 81: 2.8)  & 12\,000 & ( \  153: 4.7)  & 12\,000 & ( \ 104: 4.4)	 \\ 
\hline
$G_{\text{RVS}}<12$ & $>30$ 		& --	& 6200 & ( \quad  \ 8: 1.8)    &  7100 & ( \quad  \ 7: 1.7)  &  7300 & ( \ \ \ 21: 2.3)  & 8100 & ( \ \ \ 17: 2.3)	 \\ 
$G_{\text{RVS}}<12$ & $>50$ 		& --	& 5300 & ( \quad  \ 5: 1.8)     &  6100 & ( \quad  \ 4: 1.7)  & 6500 & ( \ \ \ 14: 2.2)  & 7300 & ( \ \ \ 12: 2.1)	 \\ 
$G_{\text{RVS}}<12$ & \ \  $>100$ 	& --	& 4300 & ( \quad  \ 3: 1.7)     &  5000 & ( \quad  \ 3: 1.7)  &  5400 & ( \quad  \ 8: 2.1)  & 6200 & ( \quad  \ 8: 2.0)	 \\ 
\hline
$G_{\text{RVS}}<12$ & --	        & $>30$     & 1700 & ( \ \ \  66: 3.1)  &  1300 & ( \ \ \  42: 3.1)  & 2700 & ( \ \ \  96: 5.2)  & 2200 & ( \ \ \  63: 4.9)  \\
$G_{\text{RVS}}<12$ & --	        & $>50$     & 1100 & ( \ \ \  55: 3.2)  &  830 & ( \ \ \  35: 3.2)  & 1900 & ( \ \ \  83: 5.2)  & 1500 & ( \ \ \  54: 5.0)  \\
$G_{\text{RVS}}<12$ & --	        & \ \ $>100$& 570 & ( \ \ \  39: 3.4)  &  410 & ( \ \ \  25: 3.4)  & 1100 & ( \ \ \  65: 5.5)  & 810 & ( \ \ \  42: 5.2) \\
\hline
$G_{\text{RVS}}<12$ & $>30$	        & $>30$     & 810 & ( \quad  \  6: 1.8)  & 750 & ( \quad  \  4: 1.8)  & 1600 & ( \ \ \  17: 2.5)  & 1500 & ( \ \ \  14: 2.4)  \\
$G_{\text{RVS}}<12$ & $>50$	        & $>50$     & 410 & ( \quad  \ 3: 1.8)  &  370 & ( \quad  \  2: 1.8)  & 950 & ( \ \ \  10: 2.3)  & 870 & ( \quad  \  8: 2.2)  \\
$G_{\text{RVS}}<12$ & \ \ $>100$	& \ \ $>100$& 140 & ( \quad  \ 1: 1.8)  &  120 & ( \quad  \ 1: 1.7)  & 400 & ( \quad  \  5: 2.3)  & 360 & ( \quad  \  4: 2.2)  \\

\hline                                             %inserts single line
\end{tabular}
\end{table*}








\begin{figure}[!htp]
%  \vspace{0cm}\\
      \centerline{\includegraphics[width=0.49\textwidth]{figures/skyDensity_lambda43.pdf} }
      \centerline{\includegraphics[width=0.49\textwidth]{figures/skyDensity_numObs.pdf} }
  %            \vspace{-0.1cm}
    \centerline{ \includegraphics[width=0.49\textwidth]{figures/typeHistLamb43.pdf} }
           \vspace{-0.1cm}
     \centerline{  \includegraphics[width=0.49\textwidth]{figures/TeffVsMassMbolLamb43.png} }
       \vspace{-0.2cm}
\caption{Distributions of the 27\,000 BDs with $\Delta \chi^2 >50$ resulting from the 5-year Ma\,\&\,Ge period distribution simulation. Top: Galactic sky density, 
second: the number of field-of-view transits for comparison with the top image, 
third: stacked histogram of stellar type (bin size:~0.2), bottom: HR-diagram and mass distribution as function of $T_{\text{eff}}$ (stellar type colour coded). To be compared to the Besan\c con input distribution of Fig.~\ref{fig:bscFig1}. \EDIT{[NOT UPDATED WITH GAIA DATA, SHOULD WE? DO we need 10 year plots as well?]} }
\label{fig:resultsTypeRelated}
\end{figure} 


\begin{figure}[!htp]
%  \vspace{0cm}\\
  \includegraphics[width=0.45\textwidth]{figures/distHist5yr.pdf} 
    \includegraphics[width=0.45\textwidth]{figures/MjupHist5yr.pdf} 
      \includegraphics[width=0.45\textwidth]{figures/semimajAxisHist5yr.pdf} 
    \includegraphics[width=0.45\textwidth]{figures/eccHist5yr.pdf} 
\caption{BD histogram distribution of the predicted 5-year \gaia mission: distance (bin size: 40~pc, top panel), BD mass (bin size: 1~M$_{\text{J}}$, second panel), semi-major axis $\overline{a}$ (bin size: 0.1~au, third panel), and eccentricity (bin size: 0.05, bottom panel). \EDIT{[not updated, I suggest to replace with some particularly relevant plots for the Ma\,\&\,Ge distribution only, perhaps for 5 and 10 year. Which plots to include? The first two, and perhaps semi-major axis versus period? ]}}
\label{fig:magHist}
\end{figure} 


%\begin{figure*}[h]
%  \vspace{0cm}\\
%  \includegraphics[width=0.49\textwidth]{figures/magHist5yr.pdf} 
%    \includegraphics[width=0.49\textwidth]{figures/magHist10yr.pdf} 
%      \includegraphics[width=0.49\textwidth]{figures/magFracHist5yr.pdf} 
%    \includegraphics[width=0.49\textwidth]{figures/magFracHist10yr.pdf} 
%\caption{BD $G$-band distribution of the predicted number of \gaia detections (top panels) and %fraction of detections per magnitude (bottom panels),  bin size: 0.5\,mag.}
%\label{fig:magHist}
%\end{figure*} 


\begin{figure*}[h]
%  \vspace{0cm}\\
  \includegraphics[draft,width=0.98\textwidth]{figures/manyAstroMa14withPhotTransits_v2}  			% MACP: remove draft
  \vspace{-0.3cm}
\caption{Distributions of the BDs resulting from the 5-yr (left) and 10-yr (right) \gaia simulation using $\textrm{P}_\textrm{distr}=$`Ma\,\&\,Ge' for the three adopted \textbf{astrometric} detection thresholds: $\Delta~\chi^2 >30$~(41\,000, 64\,000), $\Delta~\chi^2~>50$~(28\,000, 45\,000), and $\Delta~\chi^2 >100$~(17\,000, 28\,000).}
\label{fig:results1page}
\end{figure*} 

\begin{figure*}[h]
%  \vspace{0cm}\\
  \includegraphics[draft,width=0.98\textwidth]{figures/manyRvMa14withPhotTransits_v2} 				% MACP: remove draft
  \vspace{-0.3cm}
\caption{\EDIT{Same as Fig.~\ref{fig:results1page} but now for the three adopted \gaia \textbf{radial velocity} detection thresholds (i.e., limited to stars with $G_\textrm{RVS}<12$): $\Delta~\chi^2 >30$~(1700, 2700), $\Delta~\chi^2~>50$~(1100, 1900), and $\Delta~\chi^2 >100$~(570, 1100).}}
\label{fig:results1pageRv}
\end{figure*} 

\begin{figure*}[h]
%  \vspace{0cm}\\
  \includegraphics[draft,width=0.98\textwidth]{figures/manyAstroRvMa14withPhotTransits.png} 			% MACP: remove draft
  \vspace{-0.3cm}
\caption{\EDIT{Intersection of Figs.~\ref{fig:results1page} and \ref{fig:results1pageAstroRv}, i.e., where the same detection threshold is passed for both \gaia \textbf{astrometry} and \textbf{radial velocity} (hence limited to stars with $G_\textrm{RVS}<12$): $\Delta~\chi^2 >30$~(810,1600), $\Delta~\chi^2~>50$~(410, 950), and $\Delta~\chi^2 >100$~(140, 400).}}
\label{fig:results1pageAstroRv}
\end{figure*} 











